MOStream: A Modular and Self-Optimizing Data Stream Clustering Algorithm

Data stream clustering is a critical operation in various real-world applications, ranging from the Internet of Things (IoT) to social media and financial systems. Existing data stream clustering algorithms, while effective to varying extents, often lack the flexibility and self-optimization capabilities needed to adapt to diverse workload characteristics such as outlier, cluster evolution and changing dimensions in data points. These limitations manifest in suboptimal clustering accuracy and computational inefficiency. In this paper, we introduce MOStream, a modular and self-optimizing data stream clustering algorithm designed to dynamically balance clustering accuracy and computational efficiency at runtime. MOStream distinguishes itself by its adaptivity, clearly demarcating four pivotal design dimensions: the summarizing data structure, the window model for handling data temporality, the outlier detection mechanism, and the refinement strategy for improving cluster quality. This clear separation facilitates flexible adaptation to varying design choices and enhances its adaptability to a wide array of application contexts. We conduct a rigorous performance evaluation of MOStream, employing diverse configurations and benchmarking it against 9 representative data stream clustering algorithms on 4 real-world datasets and 3 synthetic datasets. Our empirical results demonstrate that MOStream consistently surpasses competing algorithms in terms of clustering accuracy, processing throughput, and adaptability to varying data stream characteristics.

==> 1_Introduction.tex <==
\section{Introduction}
\label{sec:intro}
Data stream clustering (\dsc) is a crucial operation in data stream mining, with applications in network intrusion detection~\cite{KDD99}, social network analysis~\cite{EDMStream:17}, weather forecasting~\cite{weather_forecast:2020}, and financial market analysis~\cite{cai2012clustering}. Unlike traditional batch clustering algorithms such as \kmeans~\cite{KMeans:1967,KMeans:1982} and \dbscan~\cite{DBSCAN:1996}, \dsc algorithms dynamically group incoming data based on attribute similarities and adjust clustering results upon receiving the new streaming data. \dsc algorithms must be efficient~\cite{EmpiricalR:2017,Empirical:2018}, as they are used in high-velocity environments requiring real-time decisions. Additionally, these algorithms need to address unique challenges in data stream scenarios, such as \emph{cluster evolution} and \emph{outlier evolution}~\cite{EDMStream:17,concept_evolution:2010,Concept_Evolution:10,Concept_Evolution:16,Concept_Drift_Survey:2018}, which involve the changing distribution of data and the emergence of new outliers over time and the changing dimensions of data points.

The diverse applications and performance requirements of \dsc have led to the development of numerous \dsc algorithms~\cite{BIRCH:96,Clustream:03,EDMStream:17,DenStream:06,DBStream:16,DStream:2007,SL-KMeans:20,StreamKM++:12,TSFDBSCAN:20,DenStream:06,Stream_Clustering_Survey01,Survey13}. \emph{However, these algorithms, while effective to varying extents, often lack the flexibility and self-optimization capabilities needed to adapt to diverse application contexts.} Typically, \dsc algorithms consist of four main components~\cite{wang2023sesame}: the summarizing data structure, the window model, the outlier detection mechanism, and the refinement strategy. Design choices in each component vary to meet specific needs based on application requirements, data characteristics, or performance objectives. For instance, some algorithms are optimized for processing speed~\cite{DStream:2007}, making them ideal for high-velocity data streams, while others prioritize clustering accuracy~\cite{StreamKM++:12,BIRCH:96}, a critical factor in applications requiring precise cluster assignments. The task of selecting an appropriate \dsc algorithm for real-world, diverse workloads becomes complex due to the interdependent nature of these design choices, each with its own set of trade-offs and performance implications~\cite{wang2023sesame}.


\begin{figure}[t]
	\centering
	\begin{minipage}{1\linewidth}
        \centering
		\includegraphics[width=1\linewidth]{Figures/Experiment/Motivation/Motivation_Legend.pdf}		
	\end{minipage}
	\begin{subfigure}{.245\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Experiment/Motivation/Motivation_Purity.pdf}      
         \caption{Accuracy}
         \label{fig:moti_purity}
	\end{subfigure}       
  	\begin{subfigure}{.235\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Experiment/Motivation/Motivation_Throughput.pdf}
        \caption{Efficiency}
        \label{fig:moti_throughput}
	\end{subfigure}     
        \caption{Performance comparison of nine representative \dsc algorithms and \algo on \kdd with high frequency of outlier evolution and increasing frequency of cluster evolution in the dataset.}
\label{fig:motivation}
\end{figure}


% \begin{figure}[t]
% \centering
% % \includegraphics[width=0.5\textwidth]{performance_comparison.png}
% \caption{Performance comparison of 9 representative \dsc algorithms on dynamic workloads with increasing frequency of outlier evolution.}
% \label{fig:motivation}
% \end{figure}

Figure~\ref{fig:motivation} shows the performance comparison of nine representative \dsc algorithms, including \benne~\cite{wang2023sesame}, \birch~\cite{BIRCH:96}, \skm~\cite{StreamKM++:12}, \clustream~\cite{Clustream:03}, \denstream~\cite{DenStream:06}, \dbstream~\cite{DBStream:16}, \edmstream~\cite{EDMStream:17}, \dstream~\cite{DStream:2007}, and \slkmeans~\cite{SL-KMeans:20} and our proposed algorithm \algo on \kdd with high frequency of outlier evolution and increasing frequency of cluster evolution in the dataset. We observe that both the accuracy and efficiency of existing algorithms suffer from severe degradation when processing more and more streaming data with high frequency of outlier evolution. We attribute this degradation to the inability of their static design choices to dynamically adapt to workload evolution. \benne, for example, allows manual selection of different design options for each of the four design aspects of a \dsc algorithm. While it provides a flexible framework for exploring design choices, it requires manual intervention to select the optimal configuration, which may not be practical in dynamic and rapidly changing data stream environments. In contrast, \algo\footnote{Code is at \url{https://github.com/intellistream/Sesame}} achieves highest accuracy and efficiency during the entire clustering process due to its modular and self-optimizing feature that adapts to changing workload characteristics with little overhead.

% \textbf{Novelty and Contribution.}
Similar to \benne, \algo adopts a \textbf{modular} architecture that allows flexible choices at each design aspect of \dsc algorithms and conducts a  dynamic adjustment of the modular architecture for adapting to the new worload characteristics. By further integrating dynamic adaptability, comprehensive component selection, and novel adaptation techniques, \algo effectively addresses the inherent challenges of \dsc through \textbf{self-optimizing}:
% It further achieves significant improvements over the state-of-the-art by following key innovations:

\emph{1. Dynamic Adaptability:} Unlike \benne, which uses a fixed modular configuration, \algo dynamically detects changes in workload characteristics and reconfigures itself in real-time. This capability allows \algo to maintain optimal performance under varying data stream conditions, effectively managing issues such as sudden changes in data dimensionality and outlier frequency.

\emph{2. Comprehensive Component Selection:} \algo includes an automated selection mechanism that not only considers individual component optimization but also evaluates the interplay between different design aspects (summarizing data structure, window model, outlier detection, and refinement strategy). This holistic approach ensures that the algorithm can adapt more comprehensively to diverse data stream scenarios compared to existing methods.

\emph{3. Novel Techniques for Adaptation:} \algo introduces novel techniques for flexible migration and regular stream characteristics detection, which are crucial for maintaining high performance in dynamic environments. These techniques are not present in existing algorithms like \benne and significantly enhance \algo's adaptability and efficiency.

\emph{4. Extensive Empirical Evaluations:} Through extensive empirical evaluations, \algo demonstrates superior performance in both accuracy and efficiency metrics across a wider range of datasets, including real-world and synthetic datasets with evolving characteristics. In-depth studies are also conducted to better comprehend \algo's dynamic composition capability. This breadth of evaluation underscores \algo's robustness and versatility.

Comprehensive analysis and rigorous performance evaluation with 9 representative \dsc algorithms on 4 real-world datasets and 3 synthetic datasets show that \algo consistently surpasses competing algorithms in clustering accuracy, processing throughput, and adaptability to varying data stream characteristics, including varying cluster evolution, outlier evolution, and workload dimensionality. 
% Our evaluation, spanning a wide range of real-world and synthetic workloads, validates \algo's effectiveness and generalizability. 
% Notably, \algo demonstrates superior performance in purity, CMM, and throughput metrics, particularly in scenarios characterized by high dimensionality and frequent cluster evolution.

The rest of the paper is organised as follows: Section~\ref{sec:background} introduces the background of \dsc algorithms. Section~\ref{sec:algorithm_design} discusses the algorithmic design of \algo. Section~\ref{sec:evaluation} presents our empirical evaluation of \algo. Finally, Section~\ref{sec:relatedwork} reviews additional related work, and Section~\ref{sec:conclusion} concludes the paper.

==> Acknowledgement.tex <==
\section*{Acknowledgement}
\label{sec:acknowledgement}
This work is supported by the National Research Foundation, Singapore and Infocomm Media Development Authority under its Future Communications Research \& Development Programme FCP-SUTD-RG-2022-006, and a MoE AcRF Tier 2 grant (MOE-T2EP20122-0010). Zhengru Wang and Xin Wang are co-first authors. Shuhao Zhang is the corresponding author.

==> Authors.tex <==
\author{Zhengru Wang, Xin Wang, Shuhao Zhang% <-this % stops a space
\thanks{Zhengru Wang is with Nvidia, China.}% <-this % stops a space
\thanks{Xin Wang is with the Ohio State University, USA.}% <-this % stops a space
\thanks{Shuhao Zhang is with the Nanyang Technological University, Singapore, e-mail: shuhao.zhang@ntu.edu.sg}% <-this % stops a space
\thanks{}}


% \author{Anonymous Authors}

==> Sections/3_Design.tex <==
\section{Design Components of DSC Algorithms}
\label{sec:design}
\algo modularizes the implementation of \dsc algorithms into the aforementioned four pivotal components: Summarizing Data Structure, Window Model, Outlier Detection Mechanism, and Refinement Strategy. These components collectively address the challenges and objectives outlined in the previous section. To assist in the selection of optimal design choices tailored to specific data characteristics and requirements, Table~\ref{tab:design_comparison} enumerates the advantages and disadvantages of each design aspect.

\begin{table*}[t]
\caption{Design Options in \algo}
\label{tab:design_comparison}
\centering
\begin{tabular}{|p{2.1cm}|p{2.7cm}|p{5.6cm}|p{5.7cm}|}
\hline
\textbf{Aspect} & \textbf{Option} & \textbf{Pros} & \textbf{Cons} \\
\hline
\multirow{5}{*}{Data Structure} & \CFT & Supports a range of operations & - \\
\cline{2-4}
& \CoreT & Can handle dense data streams & Involves tree rebuild \\
\cline{2-4}
& \DPT & Can handle evolving data streams & - \\
\cline{2-4}
& \MCs & Reduces computation load & - \\
\cline{2-4}
& \Grids & Computationally efficient & Limited accuracy with changing data streams \\
\cline{2-4}
& \MS & Ideal for known number of clusters & Involves sketch reconstruction \\
\hline
\multirow{3}{*}{Window Model} & \landmark & Capable of detecting drifts & Sensitive to landmark spacing \\
\cline{2-4}
& \sliding & Responsive to trends & Accuracy loss with small windows \\
\cline{2-4}
& \damped & Smooth adaptation to data evolution & Sensitive to outlier effects \\
\hline
\multirow{4}{*}{Outlier Detection} & \nod & - & May reduce clustering quality \\
\cline{2-4}
& \od & Helps improve accuracy & - \\
\cline{2-4}
& \buffer & Prevents immediate incorporation of outliers & - \\
\cline{2-4}
& \timer & Robust to outliers & Algorithm complexity \\
\cline{2-4}
& \buffertimer & High accuracy & Requires buffer time \\
\hline
\multirow{3}{*}{\shortstack{Refinement \\ Strategy}} & \norefinement & Saves computational resources & Less accurate with evolving data \\
\cline{2-4}
& \oneshotRefinement & Balances efficiency and accuracy & - \\
\cline{2-4}
& \incrementalRefinement & Adapts to new data & Computation overhead \\
\hline
\end{tabular}
\end{table*}
\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{Figures/DesignAspects/SummarizingDataStructure.pdf}
\caption{Six Types of Summarizing Data Structure in \algo.}
\label{fig:data_structure}
\end{figure}

\subsection{Summarizing Data Structure}
\label{sec:summarizing_data_structure}
In \algo, the summarizing data structure plays a critical role in providing a compact representation of the data points within the stream. This abstraction helps to enhance computational efficiency while maintaining a low memory footprint. Depending on the clustering needs, \algo offers two categories of summarizing data structures: the hierarchical category and the partitional category.

\subsubsection{Hierarchical Summarizing Data Structure}
\label{subsec:hierarchical}
Hierarchical data structures are primarily used in \algo when the data streams display inherent hierarchies or when the data can be logically grouped into a tree structure. As shown in Figure~\ref{fig:data_structure}(a), three types of hierarchical data structures are supported in \algo: Clustering Feature Tree (\CFT), Coreset Tree (\CoreT), and Dependency Tree (\DPT).

\textbf{Clustering Feature Tree (\CFT).}
\label{subsec:cf-tree}
\CFT~\cite{BIRCH:96} represents a classic yet efficient choice for hierarchical data representation in \algo. Its structure supports a broad range of basic operations required in stream clustering, such as distance calculation and cluster updating, thus providing a solid foundation for further complex manipulations.

\textbf{Coreset Tree (\CoreT).}
\label{subsec:CT}
When the data stream is characterized by high volume and density variations, \algo employs \CoreT~\cite{StreamKM++:12} to extract a core subset for processing. Despite the necessity of full tree rebuilding during clustering, which could affect efficiency, the application of \CoreT in \algo helps in obtaining high-quality clusters from dense data streams.

\textbf{Dependency Tree (\DPT).}
\label{subsec:DPT}
\DPT~\cite{EDMStream:17} is \algo's choice for handling cluster evolution effectively. The tree structure of \DPT, specifically designed to adapt to evolving activities in the stream, ensures that \algo delivers high clustering accuracy even in dynamic environments.

\subsubsection{Partitional Summarizing Data Structure}
\label{subsec:partition}
Partitional data structures, as shown in Figure~\ref{fig:data_structure}(b), are beneficial when the data streams are best represented by flat, non-overlapping clusters. In \algo, these structures are used to effectively handle and categorize incoming data points into appropriate clusters. The algorithm supports three types of partitional data structures: Micro Clusters (\MCs), Grids (\Grids), and Augmented Meyerson Sketch (\MS).

\textbf{Micro Clusters (\MCs).} 
\label{subsec:MCs}
\MCs~\cite{Clustream:03} serve as a means to reduce the computational load by representing a group of closely related data points as a single entity. With the additional elements for summarizing timestamps for clusters' updates, \MCs enable \algo to accurately track real-time clustering activities, especially under cluster evolution.

\textbf{Grids (\Grids).}
\label{subsec:Grids}
\algo uses \Grids~\cite{DStream:2007} when efficiency is paramount. The structure eliminates the need for frequent distance calculations between new data and the grid, boosting performance. Additionally, the periodic removal of sparse grids optimizes resource usage, while its fixed position may limit accuracy in cases of frequent evolving activities.

\textbf{Augmented Meyerson Sketch (\MS).}
\label{subsec:meyerson_sketch}
The \MS~\cite{SL-KMeans:20} is utilized for summarizing clustering information with a limited number of data points. Though it can be cost-intensive due to the need for sketch reconstruction to adapt to evolving data streams, it is applicable in scenarios where the exact number of clusters is known a priori. This flexibility helps \algo to accommodate diverse clustering needs.

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{Figures/DesignAspects/WindowModel.pdf}
\caption{Three Types of Window Model.}
\label{fig:window_model}
\end{figure}

\subsection{Window Model}
\label{sec:window_model}
In \algo, the window model determines the scope of the data stream that is under consideration for clustering at any given time. The selected window model influences how \algo can adapt to evolving data distributions and concept drifts. As illustrated in Figure~\ref{fig:window_model}, the three primary types of window models supported in \algo are the Landmark Window Model (\landmark), the Sliding Window Model (\sliding), and the Damped Window Model (\damped).

\subsubsection{Landmark Window Model}
\label{subsec:landmark}
In the \landmark~\cite{metwally2005duplicate}, the data stream is divided into fixed-size windows starting from a predefined landmark point. This model aids in detecting concept drifts and periodic patterns in the data by facilitating comparisons of clustering results across different windows. The primary challenge with the \landmark lies in deciding the spacing between landmarks, which has an impact on clustering accuracy and efficiency.

\subsubsection{Sliding Window Model}
\label{subsec:sliding}
The \sliding~\cite{zhou2008tracking,SL-KMeans:20} focuses on a fixed-size window encompassing the most recent data points for clustering. As new data points are processed, the oldest ones are discarded, ensuring that the algorithm remains responsive to the latest trends in the data. This model may, however, compromise clustering accuracy, particularly when the window size is small.

\subsubsection{Damped Window Model}
\label{subsec:damped}
The \damped~\cite{cao2006density,DStream:2007} assigns exponentially decaying weights to data points based on their age, giving precedence to recent data points while still considering older ones. This approach enables smoother adaptation to evolving data distributions. The \damped model is susceptible to certain stream characteristics, such as outlier effects, due to its predefined decay function parameters.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figures/DesignAspects/OutlierDetection.pdf}
    \caption{Four Types of Outlier Detection Mechanisms.}    \label{fig:outlier_detection_mechanisms}
\end{figure}
\subsection{Outlier Detection Mechanism}
\label{sec:outlier_detection}
Outlier detection mechanisms are optional design aspects in \algo that contribute to ensuring the quality of clustering results by identifying data points that deviate significantly from the overall data distribution. The two independent enhancements for this mechanism are the use of a buffer and a timer. We provide five variations, including not using any outlier detection mechanism (\nod). The other four variations are illustrated in Figure~\ref{fig:outlier_detection_mechanisms}.

\subsubsection{Basic Outlier Detection}
\label{subsec:detection}
As depicted in Figure~\ref{fig:outlier_detection_mechanisms}(a), the Basic Outlier Detection (\od) periodically identifies and removes low-density temporal clusters, improving clustering accuracy without significantly impacting efficiency~\cite{Clustream:03,DStream:2007}. Outlier detection methods can be further categorized into distance-based, density-based, and grid-based approaches, each suited to particular data stream characteristics.

\subsubsection{Outlier Detection with Buffer}
\label{subsec:buffer}
The Buffer variant (\buffer) retains potential outliers in a buffer for possible future clustering, as shown in Figure~\ref{fig:outlier_detection_mechanisms}(b)~\cite{DenStream:06,EDMStream:17}. This approach improves the overall clustering performance by keeping the temporal clusters representative of the underlying data distribution and preventing the immediate incorporation of potential outliers.

\subsubsection{Outlier Detection with Timer}
\label{subsec:timer}
The Timer variant (\timer) uses a timer mechanism, as illustrated in Figure~\ref{fig:outlier_detection_mechanisms}(c), to evaluate the activity of temporal clusters before transforming them into outlier clusters. This method enhances the robustness of the outlier detection process and the overall accuracy of the clustering results. The trade-off is an increase in algorithmic complexity and the risk of preserving noisy clusters.

\subsubsection{Outlier Detection with Buffer and Timer}
\label{subsec:buffertimer}
As depicted in Figure~\ref{fig:outlier_detection_mechanisms}(d), the combined Buffer and Timer variant (\buffertimer) retains outlier clusters in a buffer and uses a timer to evaluate their activity before transforming them into outlier clusters. Although this method improves the clustering accuracy, it increases the time required for buffer maintenance.

\subsection{Refinement Strategy}
\label{sec:refinement_strategy}
The refinement strategy, an optional design aspect, helps to maintain the adaptability of \dsc algorithms to evolving data distributions and concept drifts by updating the clustering model with new data points. Depending on computational efficiency, clustering accuracy, and adaptability to data distribution changes, there are three strategies available: \norefinement, \oneshotRefinement, and \incrementalRefinement.

\subsubsection{No Refinement}
\label{sec:no_refinement}
The \norefinement strategy, as depicted in Figure~\ref{fig:refinement} (a), outputs the temporal clusters $C$ as the final results without further refinement. This strategy saves computational resources but may lower the clustering accuracy when handling evolving data distributions or concept drifts.

\subsubsection{One-shot Refinement}
\label{sec:oneshot_refinement}
The \oneshotRefinement strategy (Figure~\ref{fig:refinement} (b)) performs model refinement less frequently to balance computational efficiency and clustering accuracy. This strategy is effective when computational resources are limited or the data stream changes gradually, allowing infrequent model updates.

\subsubsection{Incremental Refinement}
\label{sec:incremental_refinement}
The \incrementalRefinement strategy (Figure~\ref{fig:refinement} (c)) updates the clustering model continuously as new data points arrive. This keeps the model current and adaptable but may increase computational overhead. The trade-off is improved clustering accuracy at the cost of computational complexity.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/DesignAspects/OfflineRefinementStrategy.pdf}
    \caption{Refinement Strategies.}
    \label{fig:refinement}
\end{figure}


==> Sections/3_Design_OLD.tex <==
\section{Benne's Modular Design Components}
\label{sec:design}
In this section, we provide a detailed description of \algo's modular design and its components, which are organized into four key design aspects: summarizing data structure, window model, outlier detection mechanism, and refinement strategy. This modular design allows for better adaptability, configurability, and extensibility, catering to various requirements in different application domains.

\subsection{Summarizing Data Structure}
\label{sec:summarizing_data_structure}
The summarizing data structure serves as a compact representation of the data points within the stream, facilitating efficient clustering while minimizing memory and computation overhead. In \algo, we provide several options for summarizing data structures, classified into two categories: the hierarchical category and the partitional category. 

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{Figures/Design Aspects/Summarizing Data Structure.pdf}
\caption{Six Types of Summarizing Data Structure.}
\label{fig:data_structure}
\end{figure}

\subsubsection{Hierarchical Summarizing Data Structure}
\label{subsec:hierarchical}
Hierarchical summarizing data structures group the incoming data points into a tree structure. As shown in Figure~\ref{fig:data_structure}(a), each temporal cluster is depicted as a \emph{node}, and the parent cluster comprises multiple sub-clusters within the tree. To insert a new data point, it starts by searching for a suitable temporal cluster from the root node to one of the leaf nodes. Such a tree structure makes the insertion fast as there is no need for checking every existing temporal cluster. In the following, we discuss three popular and representative hierarchical summarizing data structures: Clustering Feature Tree (\CFT), Coreset Tree (\CoreT), and Dependency Tree (\DPT).

\textbf{Clustering Feature Tree (\CFT).}
\label{subsec:cf-tree}
\CFT~\cite{BIRCH:96} is one of the oldest but representative hierarchical summarizing data structures. Every tree node of \CFT is named \emph{clustering feature (CF)}, which consists of the position information of a temporal cluster. Although CF is quite simple, it is adequate to support many basic operations of stream clustering, such as distance calculation and cluster updating. Due to the additivity of the CF~\cite{BIRCH:96}, \CFT can be updated incrementally rather than starting from scratch again. Moreover, it also offers some advanced operations such as merging or splitting for handling \cef during stream clustering. \CFT captures the statistical properties of the data distribution, such as mean, variance, and density. This structure enables efficient computation of cluster distances and supports online updates as new data points are processed.

\textbf{Coreset Tree (\CoreT).}
\label{subsec:CT}
\CoreT~\cite{StreamKM++:12} is a binary tree structure used for extracting a core subset from a large volume of stream data. Compared with CF in \CFT, the tree node of \CoreT named \emph{CoreNode} provides additional information about the density of the corresponding cluster. However, since \CoreT is unable to update incrementally like \CFT, it needs to rebuild the whole tree structure during the clustering procedure, which might influence the clustering efficiency of the whole algorithm. To overcome this shortage, \CoreT reduces the time of rebuilding via lazily performing the update. In exchange, it may not be able to provide real-time clustering information for accurate clustering, especially when \cef happens frequently.

\textbf{Dependency Tree (\DPT).}
\label{subsec:DPT}
\DPT~\cite{EDMStream:17} is one of the most recent hierarchical summarizing data structures. It is specifically designed for handling \cef. The tree node of \DPT is called \emph{cluster cell} (CC), which is constructed based on cluster density. Each low-density cluster connects to its nearest denser cluster. Although CC contains similar information to CoreNode in \CoreT, it can partially adjust itself to adapt to evolving activities in the stream, achieving higher clustering efficiency.
\DPT focuses on detecting and tracking evolving density modes in the data stream, which is essential for handling \cef. By maintaining an appropriate level of cluster granularity, \DPT can efficiently adapt to the dynamic nature of the data stream, providing accurate clustering results even when \cef occurs frequently.

\subsubsection{Partitional Summarizing Data Structure}
\label{subsec:partition}
In contrast to hierarchical summarizing data structures, partitional summarizing data structures divide the incoming data points into flat clusters, as shown in Figure~\ref{fig:data_structure}(b). These clusters are non-overlapping and do not have a parent-child relationship. To insert a new data point, the partitional structures typically search for the nearest temporal cluster from the entire set of existing temporal clusters. This approach is less efficient than hierarchical structures as it requires checking all existing clusters. In the following, we discuss three typical partitional summarizing data structures, different from each other by the implementation of objects.
 
\textbf{Micro Clusters (\MCs).} 
\label{subsec:MCs}
\MCs~\cite{Clustream:03} represent a group of closely related data points as a single entity, reducing the need for maintaining individual data points in memory. A micro-cluster is defined by a set of aggregate features, such as the centroid, radius, and weight, which are updated as new data points arrive. \MCs~\cite{Clustream:03} is one of the oldest partitional summarizing data structures. It contains the same positional information as CF in \CFT. To keep track of the clusters' activities in real-time, it has two additional elements used for summarizing the timestamps for the clusters' updates. Therefore, it is more comprehensive and robust for stream clustering with high accuracy, especially under \cef.

\textbf{Grids (\Grids).}
\label{subsec:Grids}
\Grids~\cite{DStream:2007} performs its clustering simply based on checking whether the data lies in a specific grid of $d$-dimensional space and grouping the dense grids into temporal clusters. Compared to other data structures, \Grids is more computationally efficient because it does not require frequent distance calculations between new data and the grid. Additionally, it periodically removes sparse grids, which further boosts its clustering efficiency. However, since every grid has a fixed position in the space and the information about the relationship among grids is only updated lazily, \Grids may not work well when some evolving activities occur frequently among the grid and thus leads to lower clustering accuracy. \Grids partition the data space into a fixed number of cells, and each cell maintains the count of data points it contains. This approach allows for a coarse-grained representation of the data distribution, enabling efficient distance computations and outlier detection.

\textbf{Augmented Meyerson Sketch (\MS).}
\label{subsec:meyerson_sketch}
\MS~\cite{SL-KMeans:20} is the extension of traditional Meyerson Sketch~\cite{MeyersonSketch:01} which can better summarize the clustering information using a limited number of data points. \MS mainly consists of a set of temporally weighted centres, and the weight is mainly influenced by both the time and density information of the corresponding cluster. Similar to \CoreT, \MS may need to delete and reconstruct the created sketch to adapt to the evolving data stream. This brings a huge efficiency cost and temporal information loss. Another drawback of \MS is that it needs a predefined number of clusters ($K$) that is hard to determine for clustering of real-world evolving data streams.

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{Figures/Design Aspects/Window Model.pdf}
\caption{Three Types of Window Model.}
\label{fig:window_model}
\end{figure}
\subsection{Window Model}
\label{sec:window_model}
The window model defines the scope of the data stream being considered for clustering at any given time. In \algo, we support various window models, categorized into three main types as illustrated in Figure~\ref{fig:window_model}. The choice of window model affects the adaptability of the algorithm to evolving data distributions and concept drifts. Note that, for each kind of window model, there are further two types of window implementations: count-based and time-based. We base on the count-based window when implementing \dsc algorithms in our benchmark as it is more frequently used~\cite{Stream_Clustering_Survey01}.

\subsubsection{Landmark Window}
\label{subsec:landmark}
The \landmark~\cite{metwally2005duplicate} divides the data stream into fixed-size windows starting from a predefined landmark point. This model allows the detection of concept drifts and periodic patterns in the data by comparing the clustering results across different windows. As shown in Figure~\ref{fig:window_model}(a), the data between two landmarks is collected into a window for clustering. When reaching the current landmark, the temporal clustering result is stored and the current summarizing data structure is cleared. Then, the algorithm continues performing clustering based on the new 'blank' structure until reaching the next landmark. A key challenge in the landmark window model is configuring the spacing between landmarks, as this affects the clustering accuracy and efficiency.

\subsubsection{Sliding Window}
\label{subsec:sliding}
The \sliding~\cite{zhou2008tracking,SL-KMeans:20} considers a fixed-size window of the most recent data points for clustering. As new data points arrive, the oldest data points are discarded, ensuring that the algorithm focuses on the most recent trends in the data. Implemented as a queue following a First-In-First-Out processing strategy, the sliding window model, as depicted in Figure~\ref{fig:window_model}(b), maintains a predefined fixed window size. The trade-off with this approach is that, while it may reduce computation time and resources, it can also lead to decreased clustering accuracy, particularly when the window size is small.

\subsubsection{Damped Window}
\label{subsec:damped}
As shown in Figure~\ref{fig:window_model}(c), the \damped~\cite{cao2006density,DStream:2007} assigns an exponentially decaying weight to data points based on their age. This approach emphasizes more recent data points while still considering older data points, allowing for a smoother adaptation to evolving data distributions. Unlike the landmark and sliding window models, the damped window model does not treat all data objects in the window as having equal importance. Instead, it associates objects with weights that decay over time using a function $f(\alpha, \lambda)$. Additionally, the damped window model does not discard objects as time goes on, which may lead to increased accuracy but also efficiency issues. Since the $\alpha$ and $\lambda$ parameters are predefined, the decay function is kept the same to determine the priority, and the damped window model may be more susceptible to certain stream characteristics, such as \oef.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figures/Design Aspects/Outlier Detection.pdf}
    \caption{Four Types of Outlier Detection Mechanisms.}    \label{fig:outlier_detection_mechanisms}
\end{figure}
\subsection{Outlier Detection Mechanism}
\label{sec:outlier_detection}
Outlier detection mechanisms identify data points that do not conform to the underlying data distribution, which is crucial for ensuring the quality of clustering results. The outlier detection mechanism is an optional design aspect with two optional independent optimizations: the use of a buffer and a timer. In \algo, we provide five different choices for this design aspect, including not using any outlier detection mechanism (\nod).

\subsubsection{Basic Outlier Detection (\od)}
\label{subsec:detection}
The basic outlier detection mechanism (\od) periodically selects temporal clusters with low density and transforms them into outlier clusters, removing them from memory~\cite{Clustream:03,DStream:2007}, as depicted in Figure~\ref{fig:outlier_detection_mechanisms}(a). This approach can improve clustering accuracy without significantly impacting efficiency, as it reduces the number of temporal clusters, saving time for data insertion and cluster updating.

Outlier detection mechanisms can be further classified into distance-based~\cite{Clustream:03}, density-based~\cite{EDMStream:17}, and grid-based~\cite{DStream:2007} methods. Users can select the most suitable mechanism based on their specific application requirements and the nature of the data stream. 1) \emph{Distance-based outlier detection} identifies data points distant from their nearest neighbours or cluster centroids. This method is effective for detecting isolated data points and small groups of dissimilar data points in the data stream; 2) \emph{Density-based Outlier Detection} considers data points as outliers if their local density is significantly lower than that of their neighbours. This approach is suitable for detecting outliers in data streams with varying densities and complex cluster structures; 3) \emph{Grid-based Outlier Detection} uses grid-based structures to identify data points in low-density cells as outliers. This method is computationally efficient, as it relies on the grid structure for both clustering and outlier detection.

\subcompact
\subsubsection{Detection with Buffer (\buffer)}
\label{subsec:buffer}
In certain scenarios, outliers may eventually form dense clusters with other outliers, especially under the influence of \oef. To track such outliers and accommodate their potential future clustering, a buffer can be employed to store the summary of these outlier clusters for later detection (\buffer), as shown in Figure~\ref{fig:outlier_detection_mechanisms}(b)~\cite{DenStream:06,EDMStream:17}.

The buffer-based approach offers several advantages. First, it enables the clustering algorithm to better handle evolving data distributions by continuously monitoring the outlier clusters and updating their status as necessary. This allows the algorithm to be more adaptive to changes in data characteristics, improving the overall clustering performance. Second, using a buffer prevents the pollution of temporal clusters by incoming outliers. Instead of directly inserting potential outliers into the temporal clusters, they are first inserted into the outlier buffer. This ensures that the temporal clusters remain representative of the underlying data distribution and are not negatively affected by the presence of outliers.

However, maintaining the outlier buffer comes at the cost of additional computational time and resources. The buffer requires frequent updates to ensure that its contents remain relevant to the current data distribution. Moreover, the buffer may need to be periodically checked to identify and remove outdated outlier clusters or those that have become part of dense clusters.

\subcompact
\subsubsection{Detection with Timer (\timer)}
\label{subsec:timer}
In addition to using density information for periodic identification of outlier clusters, \dsc algorithms can employ a timer mechanism to evaluate the activity of temporal clusters before transforming them into outlier clusters. This approach, denoted as \timer, is illustrated in Figure~\ref{fig:outlier_detection_mechanisms}(c). The timer mechanism helps to avoid accidentally removing temporal clusters that might soon become dense and improves the overall robustness of the outlier detection process. 

The timer-based approach offers several advantages, such as:
\textit{Adaptability to dynamic data streams}: By evaluating the activity of temporal clusters based on their recent history, the timer mechanism allows the algorithm to better adapt to changing data distributions and ensure that only truly irrelevant clusters are removed.
\textit{Efficiency}: Focusing on recent cluster changes enables the \dsc algorithm to operate more efficiently, as it avoids spending computational resources on clusters that may soon become relevant again.
\textit{Improved clustering accuracy}: By preventing the premature removal of clusters that could potentially become dense, the timer mechanism improves the overall accuracy of the clustering results.

While the timer-based approach offers several advantages, it also comes with potential drawbacks that should be considered when implementing it in a \dsc algorithm: \textit{Increased complexity}: Introducing a timer mechanism can add complexity to the algorithm, as it requires additional logic to manage the timer and determine the activity of clusters. This may result in increased implementation effort and a steeper learning curve for users. \textit{Risk of preserving noisy clusters}: In some cases, the timer mechanism may inadvertently prevent the removal of noisy clusters that exhibit sporadic activity. These clusters may not be relevant to the overall data distribution but could still consume resources and affect the clustering results.

\subcompact
\subsubsection{Detection with Buffer and Timer (\buffertimer)}
\label{subsec:buffertimer}
Outlier buffer and outlier timer can be also used in combination (\buffertimer) as depicted in Figure~\ref{fig:outlier_detection_mechanisms}(d).
Similar to \buffer, \buffertimer maintains a buffer to temporarily store outlier clusters, which may transform back to temporal clusters. Different from \buffer though, \buffertimer additionally checks if a sparse temporal cluster is inactive before transforming it to an outlier cluster with the timer. Furthermore, the algorithm will also periodically check and remove some inactive outlier clusters in the buffer. This helps the algorithm improve its clustering accuracy for handling \oef but also consumes a lot of time for buffer maintenance.

\subsection{Refinement Strategy}
\label{sec:refinement_strategy}
The refinement strategy is responsible for updating the clustering model as new data points arrive and ensuring that the model remains accurate and up-to-date. This design aspect plays a crucial role in maintaining the adaptability of \dsc algorithms to evolving data distributions and concept drifts. Being another optional design aspect in \dsc algorithm, we study three design choices: \norefinement, \oneshotRefinement, and \incrementalRefinement. The choice of refinement strategy in \dsc algorithms depends on the desired trade-offs between computational efficiency, clustering accuracy, and adaptability to evolving data distributions. By carefully considering the specific requirements and characteristics of the data stream, users can select the most appropriate refinement strategy for their application.

\subsubsection{No Refinement}
\label{sec:no_refinement}
In the \norefinement approach, the algorithm directly outputs the temporal clusters $C$ as the final clustering results without any further refinement, as shown in Figure~\ref{fig:refinement} (a). This strategy is computationally efficient as it requires no additional processing but may result in lower clustering accuracy, particularly when dealing with evolving data distributions or concept drifts.

\subsubsection{One-shot Refinement}
\label{sec:oneshot_refinement}
\oneshotRefinement~\cite{StreamKM++:12, DStream:2007, DenStream:06} aims to balance computational efficiency and clustering accuracy by performing refinement less frequently, as opposed to the incremental refinement strategy. In this approach, the clustering model is refined at specific intervals or after a certain number of data points have been processed, as shown in Figure~\ref{fig:refinement} (b). While this approach can reduce the computational overhead associated with continuous updates, it may result in a less adaptive model if changes in the data distribution are not captured in a timely manner. The one-shot refinement strategy is particularly suited for applications where computational resources are limited, or when the data stream exhibits gradual changes, allowing for more infrequent model updates.

\subsubsection{Incremental Refinement}
\label{sec:incremental_refinement}
\incrementalRefinement~\cite{Clustream:03, BIRCH:96, EDMStream:17, DBStream:16, SL-KMeans:20} involves updating the clustering model on-the-fly as new data points are processed, as illustrated in Figure~\ref{fig:refinement} (c). This approach ensures that the model remains current and adaptive to changes in the data distribution but may require more frequent updates, increasing computational overhead. Some batch clustering algorithms, such as \kmeans~\cite{KMeans:1967,KMeans:1982} or \dbscan~\cite{DBSCAN:1996}, can be applied for further refining the results before output. Such a scheme is also known as the online-offline scheme and was initially proposed by \clustream~\cite{Clustream:03}. The incremental refinement strategy offers improved clustering accuracy at the cost of increased computational complexity.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/Design Aspects/Offline Refinement.pdf}
    \caption{Three Types of Refinement Strategies.}
    \label{fig:refinement}
\end{figure}

==> Sections/6_CaseStudy.tex <==
\section{Case Studies}
\label{sec:case_studies}


==> Sections/DesignAspects/3_DataStructure.tex <==
\section{Summarizing Data Structure} 
\label{sec:summarizing_data_structure}
Generally there are two main catalogues for summarizing data structure: the hierarchical catalogue and the partitional catalogue. In the following, we discuss six representative summarizing data structures commonly used in \dsc algorithms. 
Three are hierarchical-based, and three are partitional-based. Their main features is summarized in Figure~\ref{fig:data_structure}.

\begin{figure}[t] 
\centering
\includegraphics[width=0.7\textwidth]{Figures/Design Aspects/Summarizing Data Structure.pdf}
\caption{Six Types of Summarizing Data Structure.}
\label{fig:data_structure}
\end{figure}

\subsection{Hierarchical Summarizing Data Structure}
\label{subsec:hierarchical}
Hierarchical summarizing data structure groups the incoming data points into a tree structure. As shown in Figure~\ref{fig:data_structure}(a), each temporal cluster is depicted as a \emph{node}, and the parent cluster comprises multiple sub-clusters within the tree.
% Every parent node $P$ in this type of structure represents a bigger cluster and can be divided into some small sub-clusters represented by the child nodes of $P$. Therefore,
To insert a new data point, it starts by searching for a suitable temporal cluster from the root node to one of the leaf nodes. Such a tree structure makes the insertion fast as there is no need for checking every existing temporal cluster. In the following, we discuss three popular and representative hierarchical summarizing data structures different from each other for the implementation of each tree node.
% , including clustering feature tree (\CFT), coreset tree (\CoreT), and dependency tree (\DPT).


\textbf{Clustering Feature Tree (\CFT).}
\label{subsec:cf-tree}
\CFT~\cite{BIRCH:96} is one of the oldest but representative hierarchical summarizing data structures. Every tree node of \CFT is named \emph{clustering feature (CF)}, which consists of
% only consists of three elements recording 
the position information of a temporal cluster. Although CF is quite simple, it is adequate to support many basic operations of stream clustering, such as distance calculation and cluster updating. Due to the additivity of the CF~\cite{BIRCH:96}, \CFT can be updated incrementally rather than starting from scratch again. Moreover, it also offers some advanced operations such as merging or splitting for handling \cef during stream clustering.

\textbf{Coreset Tree (\CoreT).}
\label{subsec:CT}
\CoreT~\cite{StreamKM++:12} is a binary tree structure used for extracting a core subset from a large volume of stream data. Compared with CF in \CFT, the tree node of \CoreT named \emph{CoreNode} provides additional information about the density of the corresponding cluster. However, since \CoreT is unable to update incrementally like \CFT, it needs to rebuild the whole tree structure during the clustering procedure, which might influence the clustering efficiency of the whole algorithm. To overcome this shortage, \CoreT reduces the time of rebuilding via lazily performing the update. In exchange, it may not be able to provide real-time clustering information for accurate clustering, especially when \cef happens frequently.

\textbf{Dependency Tree (\DPT).}
\label{subsec:DPT}
\DPT~\cite{EDMStream:17} is one of the most recent hierarchical summarizing data structures. It is specifically designed for handling \cef.
% all types of \cef 
% as discussed in section~\ref{sec:background}. 
The tree node of \DPT is called \emph{cluster cell} (CC).
\DPT is built based on the cluster density and it requires every cluster with low density to be connected to its nearest denser cluster. Although CC contains similar clustering information as CoreNode in \CoreT, it can partially adjust itself for adapting to the evolving activities in the stream, helping to achieve a higher clustering efficiency.
% Although CC is not as flexible as CF, it additionally provides the temporal density of every cluster, helping to achieve a higher clustering accuracy, .
% can not only be used to locate the corresponding cluster but also provides the temporal density of every cluster for more precise clustering. This may lead to a higher clustering accuracy.}
% due to using more comprehensive information

\subcompact
\subsection{Partitional Summarizing Data Structure}
\label{subsec:partition}
As shown in Figure~\ref{fig:data_structure}(b), partitional
% the other catalogue of 
summarizing data structures\margi{R1O1}do not organize temporal clusters into hierarchical structures. They hence denote temporal clusters as \emph{objects}, rather than nodes.
% is based on partition, which 
% treats every cluster as an individual object instead of integrating them into a tree like the hierarchical-based one. 
When inserting a new data point, they need to check every object. This brings significant overhead compared to hierarchical structures but may help to achieve a higher clustering accuracy.
% Therefore, it will not be as efficient as the hierarchical-based one but may bring in a better clustering accuracy. 
In the following, we discuss three typical partitional summarizing data structures, different from each other by the implementation of objects.
% including micro clusters (\MCs), grids (\Grids), and meyerson sketch (\MS).


% Therefore, every time in order to find the belonging cluster for inserting the new data point, every existing cluster may have to be checked, which will bring in a more precise cluster but may also lead to a poor clustering efficiency. }
% The use of \emph{clustering feature tree} (\CFT) for summarizing large amounts of data was first introduced in the \birch algorithm. The \CFT is a very appealing summary structure for streams as it can be easily maintained online, thanks to its incremental and additive properties~\cite{Survey13}.

% As shown in Figure~\ref{fig:data_structure}(a), the \CFT is a height-balanced tree, where each non-leaf node contains at most $B$ entries, and each leaf node contains at most $L$ entries, where each entry is a CF.
% % , having each a CF and a pointer to a child node. Every leaf node contains at most $L$ entries, where each entry is a CF. 
% Each CF=($N$, $LS$, $SS$) has three components: 
% $N$, the number of data objects, 
% $LS$, the linear sum of the data objects, 
% and $SS$, the sum of squared data objects. 
% The structures $LS$ and $SS$ are n-dimensional arrays. These three components are used to compute cluster measures, such as cluster mean ($\frac{LS}{N}$), radius ($\sqrt{(\frac{SS}{N} - (\frac{LS}{N})^2)}$), and diameter ($\sqrt{(\frac{2N*SS-2*LS^2}{N(N-1)})}$).
% Each leaf node has a maximum diameter (or radius) represented by a user-defined parameter, $T$. The value of this parameter defines whether a new data object may be absorbed by a CF. Thus, $T$ determines the size of the CF-Tree, where higher values of $T$ lead to smaller trees.
 
% When a new data point arrives, it descends the \CFT from the root to the leaves by choosing in each non-leaf node its closest CF entry (closeness is defined by the Euclidean distance between new objects and the centroids of CF in non-leaf nodes). In a leaf node, the closest entry is selected and tested to verify whether it can absorb the new object. If so, the CF is updated, otherwise, a new CF is created containing this particular data point. 

\textbf{Micro Clusters (\MCs).} 
\label{subsec:MCs}
\MCs~\cite{Clustream:03} is one of the oldest partitional summarizing data structures. It contains the same positional information as CF in \CFT. To keep track of the clusters' activities in real-time, it has two additional elements used for summarizing the timestamps for the clusters' updates. Therefore, it is more comprehensive and robust for stream clustering with high accuracy, especially under \cef.
% some key characteristics such as \cef compared with \CFT.

\textbf{Grids (\Grids).} 
\label{subsec:Grids}
\Grids~\cite{DStream:2007} performs its clustering simply based on checking whether the data lies in a specific grid of $d$-dimensional space and grouping the dense grids into temporal clusters. 
% During new point insertions, density, time, and sparsity information of every grid needs to be updated. In exchange, 
Compared to other data structures, \Grids is more computationally efficient because it does not require frequent distance calculations between new data and the grid. Additionally, it periodically removes sparse grids, which further boosts its clustering efficiency. However, since every grid has a fixed position in the space and the information about the relationship among grids is only updated lazily, \Grids may not work well when some evolving activities occur frequently among the grid and thus leads to lower clustering accuracy.

\textbf{Augmented Meyerson Sketch (\MS).} 
\label{subsec:meyerson_sketch}
\MS~\cite{SL-KMeans:20} is the extension of traditional Meyerson Sketch~\cite{MeyersonSketch:01} which can better summarize the clustering information using the limited number of data points. \MS mainly consists of a set of temporally weighted centres and the weight is mainly influenced by both the time and density information of the corresponding cluster. 
Similar to \CoreT, \MS may need to delete and reconstruct the created sketch to adapt to the evolving data stream. This brings a huge efficiency cost and temporal information loss. 
Another drawback of \MS is that it needs a predefined number of clusters ($K$) that is hard to determine for clustering of real-world 
 evolving data streams.
% In order to guarantee its clustering performance for adapting to the evolving data stream, the created sketch will be frequently deleted and reconstructed, which may bring in a huge efficiency cost and temporal information loss. 
% Additionally, since the number of final clusters extracted from the sketch needs to be predefined, many representative clusters may not be kept during processing. As a result, its clustering ability will also be constrained under the evolving data stream. 

% \label{subsec:DPT}
% \DPT~\cite{EDMStream:17} is one of the most recent summarizing data structure specifically designed for handling \cef. It is constructed based on the cluster density and can handle all types of \cef as mentioned in section~\ref{sec:background}. Similar to \CFT, \DPT designs a special tree node to represent the temporal clusters, which is called \emph{cluster cell}. Although cluster cell is not as flexible as CF, it can not only be used to locate the corresponding cluster, but also stores its temporal density for building the whole hierarchical structure, which may bring in a better clustering accuracy due to using more comprehensive information.

% \subcompact
% \subsection{Micro Clusters (\MCs)}
% \label{subsec:MCs}
% A variety of \dsc algorithms use \emph{micro clusters} (\MCs) as summarizing data structures, such as \dbstream~\cite{DBStream:16}, \denstream~\cite{DenStream:06} and \clustream~\cite{Clustream:03}. 
% % The number of MC in a \MCs is specified by an input parameter $q$.
% Each \MCs contains $q$ (input parameter) MC as a list, where each MC is an extension of the CF. 

% Figure~\ref{fig:data_structure}(b) illustrates the structure of \MCs. 
% Each MC contains all three key elements (N, LS, SS) in CF, and thus can be also computed incrementally and effectively, especially under the occurrence of concept evolution. The additional components are the sum of the timestamps (LST) and the sum of the squares of the timestamps (SST). 
% Furthermore, each MC maintains a maximum boundary computed related to the mean distance of cluster objects' centroids~\cite{Survey13}.
% %constrains

% % \modify{, and each MC has a maximum
% % boundary computed related to the mean distance of cluster objects' centroids.}
% %how it works
% For each data insertion, an MC with the closest Euclidean distance is selected for potential absorption. Whether to absorb depends on 
% 1) the aforementioned maximum boundary of MC 
% and 2) the distance between the inserted data and the centroid of MC.
% A successful absorption will be followed by updating the summary statistics, or a new MC will be created otherwise.
% %clean
% The oldest MC is deleted if its timestamp is below a given threshold $\delta$ (input parameter), which is deemed to be an outlier and therefore removed. 
% We will discuss more details of outlier detection mechanisms in Section~\ref{subsec:outlier_detection_mechanism}.

% \subcompact
% \subsection{Coreset Tree (\CoreT)}
% \label{subsec:CT}
% A summarising data structure called \CoreT is proposed in the \skm algorithm~\cite{StreamKM++:12}. 
% %principle
% The key idea of constructing a \CoreT is to achieve a $\frac{1}{2}$ reduction in the number of objects by iterative expansion and summary over child nodes.

% As illustrated in Figure~\ref{fig:data_structure}(c). 
% \CoreT is a binary tree in which each node $i$ contains the following components: 
% a set of data points, $E_i$; 
% a representative point of $E_i$, $q_i$; 
% the number of data points, $N_i$; 
% and the sum of squared distances of the data points to $q_i$, $SSE_i$. 
% $E_i$ only has to be stored in the leaf nodes, because the objects of an inner node are implicitly defined as the union of the objects of its child nodes.

% \CoreT cooperates with a bucket set in \skm~\cite{StreamKM++:12} in an iterative \emph{merge-reduce} fashion. The bucket set has a finite amount of buckets and each bucket has a finite capacity of data objects, as specified in two corresponding input parameters.
% Each input data is firstly stored in a bucket of the bucket set, and the data objects in a full bucket will be moved to another bucket in the bucket set. Each pair of two full buckets will be used to construct a \CoreT for object reduction, and $\frac{1}{2}$ results will be stored in another non-empty bucket.

% in order to speed up the sampling non-uniformly during the coreset construction

% \subcompact
% \subsection{Grids (\Grids)}
% \label{subsec:Grids}
% Some \dsc algorithms such as \dstream, perform data summarization through \Grids~\cite{DStream:2007}. That is, by partitioning the n-dimensional feature space into density grid cells.  
% % Taking \dstream as an example,

% As shown in Figure~\ref{fig:data_structure}(d),
% each grid cell is represented by a tuple <$t_g$, $t_m$, $D$, $label$, $status$>.
% $t_g$ is the last time the grid cell was updated, 
% $t_m$ is the last time the grid cell was removed from the hash table that holds the valid grid cells, $D$ is the grid cell density at its last update, $label$ is the class label of the grid cell, and $status$ indicates whether the grid cell is normal or Sporadic (cells with few points are likely outliers).
% %

% % The grid cell is updated online in receiving new data and conducting data cleaning.
% % Specifically, 
% Each new input data point with $d$ dimensions is mapped to the corresponding grid cell based on the summary statistics of previous input data stored in the grid cell, then the clustering is performed based on the density of grid cells. 
% A grid cell is marked as sparse if it does not receive new objects for a long time and marked as dense otherwise. In addition, sporadic grid cells are periodically removed from the list of valid grid cells.

% the grid density is updated upon the mapping of any new input data record into the grid, and the new grid density can be updated based on the difference between the arrival time of the new data record and the last data record



% Continue to explain how clustering is performed based on the grid density...
% \subcompact
% \subsection{Dependency Tree (\DPT)}
% \label{subsec:DPT}
% The \DPT data structure is proposed by the \edmstream~\cite{EDMStream:17} algorithm. Each node in a \DPT is a \emph{cluster-cell} rather than a single point, which is for saving memory space and computation time.
% % A DP tree where each node is a cluster-cell is used to capture the summarization of data streams. 
 
% As shown in Figure~\ref{fig:data_structure} (e), a cluster-cell $c$ summarizes a group of close points, which can be described by a tuple <$s_c$, $\rho^t_c$, $\delta_c^t$> at time $t$. 
% $s_c$ is the seed point. The cluster-cell $c$ seeded by $s_c$ summarizes a set of points whose distance to $s_c$ is less than the distance to any other seed point and is less than or equal to a predefined radius $r$. $\rho^t_c$ is the summarization of all cluster-cell points' timely density at time $t$. $\delta_c^t$ is the dependent distance from $s_c$ to its nearest cluster-cell seed point with higher cluster-cell density. 
% Cluster-cells with relatively low density will not be stored in the DP tree. Instead, they are considered \emph{temporal outliers}.
% % and cached in an \emph{outlier reservoir} (Section~\ref{subsec:outlier_detec_timer}).

% Each new data point may either enter an existing data cell or lead to the creation of a new data cell to contain it. This process is distance-based and can be controlled by $r$ and $s_c$. After data insertion, the \DPT is responsible for manipulating the cluster-cells based on $t$, e.g., dependency update, emergence and decay.
% % and the time-decay value of data is therefore enabled.

% \subcompact
% \subsection{Meyerson Sketch (\MS)}
% \label{subsec:meyerson_sketch}
% The \MS data structure is initially proposed to handle online facility location problems and further extended to clustering data streams by \slkmeans~\cite{SL-KMeans:20}, which is one of the most up-to-date \dsc algorithms. 

% \MS is made up of two main elements, as shown in Figure~\ref{fig:data_structure} (f). 
% The first element is the cluster set, which stores the whole bunch of data inside the cluster and provides convenience for the algorithm to cluster the incoming data stream. However, since the data stream is infinite, it is unrealistic to store every data point in this set. Therefore, \MS gives every cluster set a unique weight decaying with time. Expired clusters are regularly deleted from the set. 
% The second element is the corresponding centre towards the cluster, which is continuously updated according to the cluster set.

% Every time when a new data point comes, \MS will use the cluster centre to calculate the cost of the whole cluster to determine whether it needs to be added to the temporal cluster. If so, it will be added to the corresponding cluster set.

\textbf{Discussion.}
\label{subsec:data_structure_discussion}
In general, hierarchical summarizing data structure improves the clustering efficiency while the partitional structure is expected to bring in better accuracy. 
The unique design of each specific structure, however, leads to further differences in their clustering behaviour.
% makes them behave differently.
% For every specific structure, their unique design and stored information 
% also influence the clustering behavior. 
For example, although \CFT, \CoreT, \DPT and \MCs promise high clustering accuracy due to the comprehensive information stored in their structure, their efficiency behaviour is quite different. Only \CFT and \DPT can guarantee high efficiency due to their flexible updating. \CoreT and \MS are slow due to frequently rebuilding the whole structure while \MCs is slow since it needs to scan every temporal cluster for data insertion. For \Grids, although it may not be as accurate as the other structures, it largely saves its computation time due to eliminating the distance calculation operation. 
% \MS requires maintaining a great number of raw data for clustering, it is hence expected to be the slowest summarizing data structure among others. 

% These summarizing data structures behave quite differently from each other in handling continuous data insertion.
% % The six summarizing data structures discussed above are all applied by \dsc algorithms to summarize and store the cluster information. During the clustering procedure, they will keep updating upon receiving a new data and utilize the stored information to insert the data into a suitable cluster. However, due to the difference in either catalog or main structure, some of them may behave quite differently from others during this common procedure. 
% {First}, 
% for hierarchical-based summarizing data structures such as \CFT, \CFT and \DPT, they do not need to check every existing cluster during data insertion.
% % clustering like those with partition-based catalog. % between parent and children nodes stored in the structure can 
% The hierarchical relationship helps them achieve a more efficient search for a suitable cluster to insert the new data point. 
% {Second},
% unlike many other summarizing data structures, \Grids does not require frequently computing the centre of clusters during data insertion. Instead, a new data point is quickly mapped to the corresponding grid cell based on the computed boundary of the cell. However, the mapping may be inaccurate or outdated overtime, leading to lower clustering accuracy. 
% % Therefore, \Grids spends much less time for data insertion. 
% % However, it leads to inaccurate data insertion and 
% % also due to the usage of boundary rather than distance, 
% % the data insertion may not be so much precise and thus \Grids may not achieve a very great clustering accuracy. 
% {Third}, 
% \MS is the only summarizing data structure that stores every data point of the cluster. Although it tries to constrain the cluster size, more time is wasted on frequently updating the centre of clusters. Moreover, due to a fixed number of clusters, the information of many historical clusters may get erased from the structure, bringing down the clustering accuracy.
% % during the clustering procedure, when more and more data is added into the stored cluster, more time will be wasted on frequently updating the center of clusters, which may result in a low efficiency. Moreover, due to the fix number of clusters, the information of many historical clusters may get erased from the structure, and this may bring down the final clustering accuracy.
% % Grid structure can ensure high efficiency but brings down the accuracy. MS may bring in a terrible clustering efficiency. Hierarchical-based summarizing data structure}

==> Sections/DesignAspects/3_Outlier.tex <==
\section{Outlier Detection Mechanism}
\label{sec:outlier_detection_mechanism}
% Our next design aspect to illustrate is outlier detection mechanism. 
Unlike the former two design aspects, the outlier detection mechanism is an optional design aspect. It further contains two optional independent optimizations: the use of a buffer and a timer, respectively. 
Put them together, including not using any outer detection mechanism (\nod), we have five different choices for this design aspect. 
% which are 1) w/o outlier detection (\nod), 2) outlier detection w/o buffer w/o timer (\od), 3) outlier detection w/ buffer (\buffer), 4) outlier detection w/ timer (\timer), and 5) outlier detection w/ buffer w/ timer (\buffertimer). 


\subcompact
\subsection{Outlier Detection (\od)}
\label{subsec:detection}
% \textbf{Outlier Detection (\od).}
As depicted in Figure~\ref{fig:outlier_detection_mechanisms}(a), 
% outlier detection refers to the process of 
% % identifying the incoming data point that is currently different from the historical ones during the clustering process. 
% %  the common and simplest way for detection is to 
% dynamically identifying the outlier clusters from the temporal ones during the clustering process. 
the basic outlier detection mechanism (\od) is to periodically select temporal clusters that are sparse in density (denoted in light colour in the figure) to transform into the outlier clusters and remove them from the memory~\cite{Clustream:03,DStream:2007}. Compared with \nod, its clustering accuracy will greatly improve. Moreover, the whole clustering efficiency may not even get influenced by adding this additional detection operation since the number of temporal clusters will be reduced, saving time for future data insertion and cluster updating.
% To achieve better outlier detection accuracy and efficiency, we discuss two common optimizations in outlier detection including the buffer and timer mechanisms in the following.
% to illustrate the use of a buffer and a timer 
% Here we only discuss the former two since they are the most popular ones.


% removing some of the real clusters from the summarizing data structure according to their updated timestamps. 
% % Introduce two outlier detection mechanisms
% Apart from identifying outliers based on density, many \dsc algorithms groups outlier objects into clusters for the convenience of transformation between outliers and real data points through two optional optimization techniques: \emph{outlier buffer}, which stores outlier candidates for further transformation; and \emph{outlier timer}, which maintains a timer for each real cluster to record the timestamps of receiving the latest data object. 
% Not every \dsc algorithm applies outlier detection to their algorithm procedure. For those using this design aspect, they 
% % the process to identify an incoming data that does not belong to any of the temporal clusters.
% Not every \dsc algorithm applies outlier detection to their algorithm procedure. For those using this design aspect, their methods are either based on distance or density as illustrated in Figure~\ref{fig:outlier_detection}.
% \tony{
% --Overview--
% Outlier detection is based on density, which is much more complex and requires more computational resources compared with distance-based one. In density-based outlier detection, density $N_0$ around a incoming data point $P$ is compared with the density around its neighboring clusters $\{N_1, N_2, N_3\}$. If the local density is much lower than the surrounding, then $P$ will be treated as an outlier.
% -- Add buffer and timer overview here ---
% }

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.38\textwidth]{Figures/Design Aspects/Outlier_Detection_Overview.pdf}
% \caption{Outlier Detection Overview.}
% \label{fig:outlier_detection}
% \end{figure}
% % The other type of 

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Design Aspects/Outlier Detection.pdf}
    \caption{Four Types of Outlier Detection Mechanisms.}    \label{fig:outlier_detection_mechanisms}
\end{figure}

\subcompact
\subsection{Outlier Detection with Buffer (\buffer)}
\label{subsec:buffer}
Due to the influence of \oef, some outliers, which can be grouped into sparse clusters with other outliers, need to be tracked during the clustering procedure. This is because these outlier clusters may become dense enough after adding more and more outliers and will be transformed into 
temporal clusters. In this case, setting a buffer to store the summary of these outlier clusters for later detection (\buffer), as shown in Figure~\ref{fig:outlier_detection_mechanism}(b), is one of the most commonly used optimization strategies in outlier detection~\cite{DenStream:06,EDMStream:17}. 
Another advantage of applying a buffer for detection is that incoming data once detected as outliers are immediately inserted into the outlier buffer rather than temporal clusters avoiding pollution. However, maintaining the outlier buffer consumes additional computational time and resources. 
% In this way, the algorithm's ability for handling \cef will not get influenced by polluting the temporal clusters with some outliers. Although preserving these outliers helps the algorithm handle the potential evolving activities and improve its clustering accuracy, maintaining the whole buffer during the clustering procedure may consume a lot of computational time and resources. 


% Since the initial proposal in the \denstream algorithm~\cite{DenStream:06}, some recent \dsc algorithms such as \edmstream~\cite{EDMStream:17} choose to create a buffer for storing temporal outliers. Due to the influence of concept evolution in a data stream, the temporal outlier clusters are required to be tracked during the clustering procedure so that they can be modified as clusters if they become dense enough after adding more and more ``outliers''. 

% The key idea is shown in Figure~\ref{fig:outlier_detection_mechanisms}(a). 
% If the incoming data point is far from any of the current clusters, it will be considered to join one of the outlier clusters inside the buffer. In this way, the density of the outlier clusters also keeps changing during the clustering procedure. 
% When some of them become dense enough, they will be removed from the buffer and be appended to the current summarizing data structure as clusters. 

% % It maintains two types of micro-clusters: \emph{p-microclusters} and \emph{o-microclusters}. 
% % The \emph{p-microclusters} keep the statistical summary of data stream during the online phase. The algorithm periodically transforms \emph{p-microclusters} to \emph{o-microclusters} whose weight are below the threshold, and store them inside the outlier buffer. To avoid memory usage overhead, only the \emph{o-microclusters} whose weight increases over time are kept in the buffer, and they will be transformed back to \emph{p-microclusters} if their weight becomes higher than the threshold.

% There are also some \dsc algorithms, such as \clustream~\cite{Clustream:03} and \dstream~\cite{DStream:2007}, do not utilize \buffer. Instead, they periodically select sparse clusters as the outlier cluster and remove them from the summarizing data structure. 
% in a regular time.

\subcompact
\subsection{Outlier Detection with Timer (\timer)}
\label{subsec:timer}
% The other popular optimization is timer. 
% which maintains \emph{outlier timers} for each cluster to identify outliers.
% In order to identify the outlier more precisely, the other popular optimization is using timer as another criteria besides density for detection. Specifically, during the clustering procedure,
Apart from periodically identifying outlier clusters via density information, \dsc algorithms may further check whether the temporal clusters are not active anymore before transforming them to outlier clusters with a timer (\timer) as illustrated in Figure~\ref{fig:outlier_detection_mechanism}(c). 
Using a timer makes the detection more robust than \od since it helps to prevent accidentally removing temporal clusters that may soon become dense.
% it requires the outlier identification based on one more criterion apart from density. 
Additionally, using a timer helps the \dsc algorithm to be more focused on the recent cluster changes, thus bringing higher efficiency.

% is suitable for the evolving data stream since it split those inactive clusters from the temporal ones and helps the \dsc algorithm to be more focused on the recent cluster changes. Moreover, it may bring in better efficiency as fewer clusters are left for further clustering.
% In this case, they will maintain an outlier detection timer in each temporal cluster to record the timestamp of the latest update.
% as depicted in Figure~\ref{fig:outlier_detection_mechanisms}. 
% For algorithms using outlier timer but not using outlier buffer (\timer), which is shown in Figure~\ref{fig:outlier_detection_mechanism}(c), only the temporal clusters that are not only sparse but also inactive will be treated as outlier clusters and get removed from memory. 

\subcompact
\subsection{Outlier Detection with Buffer and Timer (\buffertimer)}
\label{subsec:buffertimer}
Outlier buffer and outlier timer can be also used in combination (\buffertimer) as depicted in Figure~\ref{fig:outlier_detection_mechanism}(d).
% However, if using outlier timer in combination of outlier buffer (\buffertimer), as depicted in Figure~\ref{fig:outlier_detection_mechanism}(d), 
Similar to \buffer, \buffertimer maintains a buffer to temporarily store outlier clusters, which may transform back to temporal clusters. Different from \buffer though, \buffertimer additionally checks if a sparse temporal cluster is inactive before transforming it to an outlier cluster with the timer. Furthermore, the algorithm will also periodically check and remove some inactive outlier clusters in the buffer. This helps the algorithm improve its clustering accuracy for handling \oef but also consumes a lot of time for buffer maintenance.
% The algorithm will instead insert the sparse and inactive temporal clusters into the buffer and check whether some of the outlier clusters become dense enough to be transformed into temporal clusters. 
% Moreover, 
% \tony{Possibly, using buffer and timer together for outlier detection will synthesize both their pros and cons, making this operation more comprehensive and robust.}
% for real clusters which are stored in summarizing data structure, at every regular interval, only those which are not only sparse in density (below $D$) but also inactive in timer (above $T$), will be regarded as outlier clusters and get removed or thrown into the buffer (if the buffer is used). 
% Similarly, outlier clusters stored in the buffer will also get removed if being regularly checked as inactive (above $T$).  
% When some of the sparse clusters are inactive for a long time, they will be regarded as outlier clusters or thrown into the buffer (if the buffer is used) as depicted in Figure~\ref{fig:outlier_detection_mechanisms}. 
% Compared with detecting outliers merely based on density, including \od and \buffer, 


% Algorithms such as \birch, keep identified outliers till the end of processing.
% Some other \dsc algorithms, such as \clustream~\cite{Clustream:03}, \dstream~\cite{DStream:2007} and \edmstream~\cite{EDMStream:17} propose 
% outlier detection w/ timer (\timer).
% Specifically, they maintain \emph{outlier timers} for each cluster to identify outliers. 
% The cluster timestamp will be renewed each time upon the arrival of a new data object, clusters with outdated timestamps might be removed from the summarizing data structure. 

% As depicted in figure~\ref{fig:outlier_detection_mechanisms}(b), each cluster maintains a timer to record the timestamp of the latest update.
% % the other metric that many \dsc algorithms, such as \clustream~\cite{Clustream:03}, \dstream~\cite{DStream:2007} and \edmstream~\cite{EDMStream:17} apply to detect outliers is setting the timer for every real cluster. 
% When some of the clusters are always in low density for a long time, they are regarded as outlier clusters.
% % and either be removed from the memory or put into the outlier buffer if utilized. 
% When used together with an outlier buffer, this detecting metric can also help the buffer to regularly delete some of its old and sparse clusters for keeping the buffer size within an acceptable range to improve clustering efficiency. 
% Although maintaining timers increases memory footprints and brings in additional overhead, it helps \dsc algorithms to identify outliers in a more comprehensive manner. 

\textbf{Discussion.}
The buffer and timer optimizations can be applied either separately or simultaneously, resulting in different decisions regarding the outlier detection mechanism. 
% However, their main contribution to the final clustering behaviour is not the same. Specifically, 
The use of a buffer can greatly improve the clustering quality due to its better ability for handling \oef. However, maintaining the outlier buffer in real-time will also bring down the efficiency. 
On the contrary, the use of the timer may be beneficial for both better clustering accuracy and efficiency, especially under \oef. 
Using a buffer and timer together in outlier detection further complicates the clustering behaviour and motivates an in-depth study.
% the impact of the timer towards the clustering behaviour is less significant compared to the use of a buffer, but it 
% In most cases it is beneficial 


% Both two outlier detection mechanisms can contribute to better clustering behaviour but their contributions are quite different.
% \underline{First}, 
% buffers can be used to track the changes of temporal outliers in the stream, and they help to improve clustering accuracy, especially under varying workload characteristics. However, maintaining the outlier buffers brings significant performance overheads.
% \underline{Second}, 
% timers help to remove temporal clusters and improve clustering efficiency as a result. 
% However, its impact on clustering accuracy is rather non-deterministic as it brings in a more sophisticated deletion process of outdated clusters.
% rather than storing them in the buffer.
% for detecting with buffer, since it can be used to track the changes of temporal outliers in the stream, this design selection can greatly improve the accuracy and thus indirectly improve its adaptability under varying workload characteristics. 
% However, due to the requirement for frequently maintaining the outlier buffer, the clustering efficiency will decrease a lot.

% For detecting with timer, its improvement on clustering accuracy is not as very large because it only brings in a more sophisticated and reasonable deletion of outdated clusters rather than storing them into the buffer. However, when more and more clusters are required to be deleted, the number of temporal clusters will decrease a lot and the total clustering efficiency will eventually get improved.

% This will severely impact the whole clustering efficiency if growing to large. 

% timer records the last timestamp for updating the current cluster.
% and will be renewed after adding a new data point. 

% Although frequently maintaining the timer for the real clusters will increase the memory footprint and bring in additional time consumption during the execution, it will help the \dsc algorithm to identify the outliers with a more comprehensive way. That is, when some of the real clusters are always in low density, they should also be regarded as outlier clusters and either be removed from the memory or put into the buffer. Also, when being used with buffer, this detecting metric can also help the buffer to regularly delete some of its old and sparse clusters for keeping the buffer size into an acceptable range, which will severely impact the whole clustering efficiency if growing to large. 

% \tony{Who didn't apply timer? Add the discussion here.}
% Many \dsc algorithms apply timer into their outlier detection mechanism. Some exceptional cases exist. 
% % however, there are also some exceptional cases. 
% For example, algorithms such as \birch do not consider timer for detecting outlier in the stream. For these algorithms, after inserting the new outlier into the clusters, they will keep these outliers till the end of processing and then directly remove those still in low density from the memory.

% Both of the two former types need to find the nearest cluster $C_1$ of the input data. After that, distance-based methods use the distance between input data and $C_1$ while density-based methods directly check the density of $C_1$ to judge whether the input data is an outlier. Different from the two former types, buffer-based outlier detection gives every input data a unique weight changed with time and stores those temporal outliers into an outlier buffer. Moreover, buffer-based outlier detection periodically checks the weight of points to see whether some of the cluster points have become outliers or some of the outliers in the buffer have converted into the cluster points. 
% instance that seems to be different from the remaining of the data. 
% Upon a new data coming, it will be discarded into the outlier buffer if it does not belong to any of the clusters, or it belongs to a cluster whose cardinality is far less than other clusters. Outlier detection metrics are also helpful for handling concept evolution, especially for the emerge type of concept evolution. It is possible that some of the historical points in the outlier buffer are becoming connected with others and should be grouped into a new cluster in the current timestamp.


% https://tex.stackexchange.com/questions/9584/how-to-put-subfigures-in-several-rows @Zhonghao

% \begin{figure}
% \centering
% \begin{tabular}{cc}
% \subfloat{
%     \centering
%     \includegraphics[width=.48\linewidth]{Figures/Design Aspects/Outlier_Buffer_Label.pdf}
%     } &
% \subfloat{
%     \centering
%     \includegraphics[width=.48\linewidth]{Figures/Design Aspects/Outlier_Timer_Label.pdf}
%     }
% \end{tabular}
% \caption{Outlier Detection Mechanisms}\label{outlier_detection_mechanisms}
% \end{figure}

% \begin{figure}[htbp]
%     \subfloat{
%     \begin{minipage}[t]{0.44\linewidth}
%         \centering
%         \includegraphics[width=1\linewidth]{Figures/Design Aspects/OutlierBuffer.pdf}
%         \label{fig:outlier_buffer}
%         \caption{Outlier Buffer}
%     \end{minipage}
%     }\hfill
%     \subfloat{
%         \begin{minipage}[t]{0.44\linewidth}
%         \centering
%         \includegraphics[width=1\linewidth]{Figures/Design Aspects/Outlier_Detection_With_Timer.pdf}
%         \caption{Outlier Timer}
%         \label{fig:outlier_timer}
%     \end{minipage}
%     }\tony{Change to subfloat.}
% \end{figure}


% It is impractical to store the entire input data, not only because data streams are infinite, but also because the process of handling concept evolution will be hampered. 
% It further consists of three key components: primitive data structures, global data structures, and the supported operations.
% % usually consists of two categories in stream clustering, namely primitive data structures and global data structures. 
% 1) 
% Primitive data structure refers to the basic structure that summarizes the stream in order to preserve the meaning of the original objects without the need of actually storing them. 
% Common primitive data structures include micro-clusters (MCs) and grids. 
% A variety of DSC algorithms use MC as a primitive data structure, such as BIRCH~\cite{BIRCH:96}, ClusTree~\cite{Clustree:2011}, DenStream~\cite{DenStream:06} and Clustream~\cite{Clustream:03}. 
% It maintains distribution information for a group of gathered data objects. 
% Grid is a data structure formed by partitioning the n-dimensional feature space into density grid cells. Summary statistics are maintained for all objects that are mapped to the corresponding grid cell.
% 2) Global data structure refers to the structure made up of the elements in primitive data structure. It mainly functions to provide relationships between these elements for further supported operations.
% \tony{
% --seems wrong---
% 3) Supported operation refers to which kinds of concept evolution mentioned in Section~\ref{sec:2.1} the corresponding DSC algorithm can deal with. It is possible that algorithms with different key design aspects can handle different concept evolution.
% }


==> Sections/DesignAspects/3_Refinement.tex <==
\section{Offline Refinement Strategy}
\label{sec:offline_refinement_strategy}
% \tony{Messy. Unreadable. Clean it up.}
The basic idea of the offline refinement strategy is to utilize offline clustering algorithms to improve the online clustering results.
% is to apply some offline clustering algorithms to refine the clustering results from stream clustering. 
Being another optional design aspect in \dsc algorithm, we study two design choices, \norefinement and \refinement.
As shown in Figure~\ref{fig:offline_refinement_strategy}, if apply \norefinement, the algorithm will directly output the temporal clusters $C$ as the final clustering results.
Instead, if \refinement is applied, some batch clustering algorithms, such as \emph{density-based} (\dbscan) or \emph{distance-based} (\kmeans), will be applied on $C$ for further refining the results before output. 
% Although it can be classified according to different types of offline clustering algorithms, such as \emph{density-based} (\dbscan) or \emph{distance-based} (\kmeans). Here we only consider two general conditions, which are \norefinement and \refinement. 
% , otherwise some tradit
% ional clustering algorithms will be applied on $C$ for further refining the results before output, which is denoted as \refinement. 


\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{Figures/Design Aspects/Offline Refinement.pdf}
    \caption{Offline Refinement Strategy.}
    \label{fig:offline_refinement_strategy}
\end{figure}

% Similar to the outlier detection mechanism, offline refinement strategy is an optional design aspect for building a \dsc algorithms. Various \dsc algorithms, such as CluStream~\cite{Clustream:03} and DenStream~\cite{DenStream:06} utilize a distance-based or density-based offline clustering algorithm to refine their stream clustering results only once. 

% The key idea of offline refinement strategy is illustrated in figure~\ref{fig:Offline-Refinement}(a). It mainly functions to apply some traditional clustering algorithms such as \kmeans~\cite{KMeans:1967,KMeans:1982} or \dbscan~\cite{DBSCAN:1996} to refine the stream clustering results. Such a scheme is also known as the online-offline scheme and was initially proposed by \clustream~\cite{Clustream:03}. 
% %  optimize the stream clustering results by using 
% % \dsc algorithms often adopt the ``two-phase scheme'' framework to process the infinite data streams, which is proposed in~\cite{Clustream:03}. 
% %
% The \emph{online component} evaluates input data points in real-time and captures relevant summary statistics of the observations. The online evaluation result is a number of \emph{micro-clusters} representing a large number of preliminary clusters in the input data stream.
% %
% As shown in figure~\ref{fig:Offline-Refinement}(b), the \emph{offline component} uses the micro-clusters to derive the final clustering, so-called macro-clusters. This process is also called reclustering and is usually not considered time-critical which allows employing variants of traditional clustering algorithms.
% % Different from the other three design aspects discussed above, 
% % Offline refinement can be executed at offline stages in \dsc algorithms 
% Specifically, after finishing stream clustering, algorithms can run offline clustering on those final updated primitive data structures $\{D_1, D_2, ..., D_q\}$ to get the further refinement clusters $\{C_1, C_2, ..., C_m\}$. In most cases, $q$ is much bigger than $m$ and thus this step can also be regarded as a way for handling \emph{merge} type of \cef.

\textbf{Discussion.}
Offline refinement is optional and can be easily applied to refine online clustering results before outputting the result. The common wisdom is that it may further improve clustering quality.
% , but bring some performance overheads.
Unfortunately, there is no prior study about the real impact of this design aspect on both accuracy and efficiency. Even in recent years, some choose~\cite{StreamKM++:12} to involve this design aspect in their proposed \dsc algorithms, and some choose not~\cite{EDMStream:17}. We will empirically show its impact via extensive evaluations.
% Therefore, it is still an unloving problem about when and how to use this design aspect for a better clustering behavior.
% The true function of this design aspect is to improve the final clustering quality via some traditional clustering algorithms, which are often either based on distance or density. Since in most cases we may only obtain the clustering centers as the final result, this design aspect is optional and can be easily applied to refine these centers before outputting the result. However, due to the fact there are still a great number of \dsc algorithms which do not use this design aspect, its true impact and meaning towards the clustering behavior is still doubtful.
% \tony{A few algorithms periodically apply offline refinement to incrementally updates online clustering results, such as EDMStream~\cite{EDMStream:17}. -- Double Check -- If yes, update the table 2: one-time-only vs periodical.}

% \begin{figure}[t]
%     \begin{subfigure}[t]{0.23\textwidth}
%       \includegraphics[width=\linewidth]{Figures/Design Aspects/online-offline.png}
%       \caption{Online-Offline framework}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.23\textwidth}
%       \includegraphics[width=\linewidth]{Figures/Design Aspects/refinement stage.pdf}
%       \caption{Offline Refinement Process}
%     \end{subfigure}
%     \caption{Offline Refinement}
%     \label{fig:Offline-Refinement}
% \end{figure}
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 

==> Sections/DesignAspects/3_Window.tex <==
\section{Window Model} 
\label{sec:window_model}
% In order to cluster the evolving data stream in a more efficient way, it is better to only process recent data rather than the whole one. 
% In most cases, more recent information from the stream can reflect the changes in temporal clusters. Thus, this information can be used to detect and explain the evolution of the process under observation, which can improve the algorithm's ability to handle the evolving data stream. 
% To this end, the window model is used to determine the most recent input data for processing. 
The window model can be categorized into three main types as illustrated in Figure~\ref{fig:window_model}. 
% They are landmark (\landmark), sliding (\sliding), and damped (\damped) window models respectively.
For each kind of window model, there are further two types of window implementations: count-based and time-based. 
% Following prior works~\cite{Stream_Clustering_Survey01}, 
We base on the count-based window when implementing \dsc algorithms in our benchmark as it is more frequently used~\cite{Stream_Clustering_Survey01}.


\begin{figure}[t]
\centering
\includegraphics[width=0.7\textwidth]{Figures/Design Aspects/Window Model.pdf}
\caption{Three Types of Window Model.}
\label{fig:window_model}
\end{figure}

\subcompact
\subsection{Landmark Window Model (\landmark)}
\label{subsec:landmark}
% The \landmark handles objects in the form of disjoint portions of the data stream, which is separated by relevant objects such as the time-point or the number of objects observed in the previous window. 
% All objects that arrived after the landmark are considered as part of the current window until the next landmark is reached. When a new landmark is reached, all objects in the previous window are discarded, only those arriving after the new landmark are processed. 
As shown in Figure~\ref{fig:window_model}(a), \landmark collects the data between two landmarks into a window for clustering. When reaching the current landmark, the temporal clustering result will be stored before clearing the current summarizing data structure. After that, the algorithm will continue performing clustering based on the new `blank' structure until reaching the next landmark. 
It is hard to define a proper landmark configuration for \landmark.
% The key challenge of \landmark is that . 
If the two landmarks are spaced very close together, many evolving activities in the stream will not be captured inside the window, leading to poor clustering accuracy. On the contrary, if the two landmarks are set far from each other, a great number of data points will be involved inside the window for computation and the efficiency will decrease significantly.


\subcompact
\subsection{Sliding Window Model (\sliding)}
\label{subsec:sliding}
\sliding is usually implemented as a queue following a First-In-First-Out processing strategy as depicted in Figure~\ref{fig:window_model}(b).
% stores the most recent objects in \change{the window with a predefined window size}
% a data structure, whose size is fixed and defined at the beginning. 
% , where the first object entering the window will be the first one to exit. 
Similar to the \landmark, the \sliding only considers data objects whose timestamp falls within the current window range with older ones discarded. 
In contrast to the \landmark whose window size can be dynamically determined by the landmark, the size of the \sliding is predefined with a fixed value.
% it is usually employed in scenarios when we are only interested in the most recent objects. 
The non-discriminate nature of data insertion and deletion results in a smaller number of clusters by comparison and thus reduces computation time and resources. However, this also means the clustering accuracy will greatly decrease especially under a small window size configuration.
% will be affected by the presence of outliers and \cef in the stream.

% On the contrary, the length of the \sliding needs to be set at the very beginning and will not be changed any longer. Every time when new $k$ points arrive, they will be immediately inserted into the window and the window will also discard its first $k$ points for keeping the length unchanged. 

\subcompact
\subsection{Damped Window Model (\damped)}
\label{subsec:damped}
For both the \landmark and the \sliding, all data objects in the window are associated with equal importance. In contrast, to\margi{R1O1}ensure the more recent data points in the window are always being treated with higher priority, the \damped associate objects in the data stream with weights that decay with a function $f(\alpha, \lambda)$ over time. Meanwhile, unlike the other two types of window models, \damped does not discard objects as time goes on. While taking all data into account may bring in high accuracy, this causes efficiency issues. Furthermore, since the $\alpha$ and $\lambda$ parameters are predefined, the decay function is always kept the same to determine the priority, and the \damped may be more susceptible to some stream characteristics such as \oef.
% Add some discussions of the periodical update process under \damped. 
\begin{comment}
\tony{Notably, some existing algorithms with \damped such as \dstream~\cite{DStream:2007} assume that only one data comes in every time unit. In this case, they only need to update the weight once within a computed time gap, which may greatly improve its efficiency. However, since the gap value is determined by the current number of clusters, this profit may disappear after processing more and more evolving data stream.}
\end{comment}

% In contrast, the \damped associates objects in the data stream with weights that decrease over time, which are usually determined by decay functions. 
% % One typical decay function used for the \damped is the exponential decay function: 
% % \(f(t) = 2^{-\lambda(t_c-t_o)}\), where \(t_c\) is the current time point and \(t_o\) is the creation time. 
% This ensures the most recent information in the data stream is always treated with higher priority. 
% % Different from landmark and sliding window, 
% The \damped does not discard objects as time goes on. Instead, it gradually reduces their significance by associating them with lower weights. While taking all data into account ensures a good level of accuracy, this causes efficiency issues. Furthermore, it is more susceptible to the frequency of evolution and the number of outliers in the data stream.

% Density window model gives every input data a unique weight decaying with time to ensure those most recent data being treated with priority. Landmark and \sliding both similarly collect a bunch of most recent data into a window buffer and use window length and time difference respectively to determine whether to process the collected data using \dsc algorithms.
% In most cases, the recent information from the stream can reflect the changes of temporal clusters. Thus, this information can be used to detect and explain the evolution of the process under observation, which can improve the algorithm's ability to handle the evolving data stream.
% Only when the current window is full will DSC algorithms be executed. 
% Currently, there are three main kinds of window models, they are landmark, sliding and damped window \wangxin{model} respectively.

\textbf{Discussion.}
% Although the three types of window model can all be applied to keep the most recent data from the stream, the different window length makes their clustering behaviour quite different from others. 
Although these window models all try to prioritize the most recent data from streams, their specific strategies are quite different leading to different clustering behaviours. For a better clustering efficiency, \sliding may be the best choice since its fixed window size largely reduces the number of clusters for maintenance. On the contrary, although both \landmark and \damped may not be as efficient as the \sliding, they can bring in more accurate clustering results. Finally, for all three types of window models, their clustering behaviour is sensitive to their specific window configurations, which have not been studied in depth in the literature.
% {First}, the \landmark and \damped have no constraint on their window length, retaining much more information than the \sliding. They essentially bring a tradeoff between accuracy and efficiency. The more information retained, the higher the accuracy, and the lower the efficiency.
% {Second}, it can be a difficult task to set correct window configurations. For the \landmark, it is hard to determine the best landmark. While for the \damped, its decaying function has fixed parameters and can not be adaptive to varying workload characteristics.

% Specifically, as discussed before,\sliding can be helpful to improve the clustering efficiency but may lower the total accuracy. On the contrary, for landmark and damped window model, since they have no constraint on their window length, their clustering accuracy is higher than the sliding one. However, their infinite length of window may also bring in a terrible efficiency problem. Additionally, for \landmark, it is difficult to determine the best landmark. For the damped window model, its usage of decaying function may also damage the original clustering information, which makes itself more susceptible to varying workload characteristics.

==> Sections/Model_bk.tex <==
\section{\algo's Algorithm Design}
\label{sec:selection}
% In this section, we propose an automatic option selection mechanism to guide users in selecting suitable options for Benne. The mechanism consists of four functions that help users choose the most appropriate summarizing data structure, window model, outlier detection mechanism, and refinement strategy based on their primary performance objective and input data stream characteristics. The primary performance objective can be Accuracy, Efficiency, or Balance.
In this section, we discuss the completed algorithm design of \algo. Through flexible adaptability among varying design choices based on the varying stream workload characteristics and user-defined optimization targets, \algo can better utilize the advantages of every different design choices and thus guarantee a better clustering behavior under the specific optimization target.

\subsection{Workflow of \algo}
The \algo algorithm follows a two-phase execution strategy: online phase and offline phase. The adaptability of \algo comes from the configurability of its components, including the summarizing data structure ($struc.$), window model ($win.$), outlier detection mechanism ($out.$), and refinement strategy ($ref.$). According to the evolving stream characteristics detected from the collected stream samples $queue$ and with the predefined threshold values $thresholds$, This adaptability allows \algo to cater to the specific needs of various applications and data streams.
Algorithm~\ref{alg:algo} presents the high-level execution flow of \algo. 

During the online phase, the algorithm processes the input data stream by following these steps:
\emph{Window Function} (Line 2): The \texttt{Window Fun.} manages the data points in the summarizing data structure ($s$) according to the selected window model ($win.$). This function ensures that the clustering process focuses on the most relevant data points and adapts to the evolving data distributions.
\emph{Outlier Detection} (Lines 3-7): If the outlier detection mechanism ($out.$) is enabled, the \texttt{Outlier Fun.} is invoked to determine whether the current input point ($p$) is an outlier. If the point is not an outlier, it is inserted into the summarizing data structure ($s$) and updated it accordingly (Line 6). If the outlier detection mechanism is not enabled, the input point is directly inserted into the summarizing data structure (Line 8).
\emph{Incremental Refinement} (Lines 9-10): If the refinement strategy ($ref.$) is set to \incrementalRefinement, the algorithm performs the \texttt{Refine Fun.} as new data points are processed. This approach ensures that the clustering model remains up-to-date and adaptive to changes in the data distribution but may require more frequent updates, increasing computational overhead.

After processing the entire input data stream, the algorithm enters the offline phase:
\emph{One-shot Refinement} (Lines 11-12): If the refinement strategy ($ref.$) is set to \oneshotRefinement, the algorithm performs the \texttt{Refine Fun.} in a single pass at the end of the stream processing. This approach reduces the computational overhead by performing refinement less frequently but may result in a less adaptive model if changes in the data distribution are not captured in a timely manner.
By setting different types of $struc.$, $win.$, $out.$, and $ref.$, the \algo algorithm can be easily reconfigured into various variants, allowing it to adapt to different scenarios and data stream requirements.

% \begin{algorithm}[h]
% \scriptsize
% \caption{Execution flow of \algo.}
% \label{alg:algo}
%     \KwData{$p$ \tcp{Input point}}
%     \KwData{$s$ \tcp{Summarizing data structure}}
%     \SetKwInput{KwData}{Input}
%     \KwData{$struc.$ \tcp{Selected type of summarizing data structure}}   
%     \KwData{$win.$ \tcp{Selected type of window model}}
%     \KwData{$out.$ \tcp{Selected type of outlier detection mechanism}}
%     \KwData{$ref.$ \tcp{Selected type of refinement strategy}}
%     \tcp{Online Phase}
%     \While{!stop processing of input streams}{
%         \texttt{Window Fun. (...)}\;
%         \eIf{\text{$out.$ != \nod}}{
%             $b$ $\gets$ \texttt{Outlier Fun. (...)}\;
%             \If{\text{$b$ = false}}{
%                 \texttt{Insert Fun. (...)\tcp{Insert $p$ to $s$ and update $s$}}            
%             }
%         }{
%             \texttt{Insert Fun. (...)\tcp{Insert $p$ to $s$ and update $s$}}
%         }
%         \If{\text{$ref.$ = \incrementalRefinement}}{
%             \texttt{Refine Fun. ($ref.$)};
%         }
%     }
%     \tcp{Offline Phase}
%     \If{\text{$ref.$ = \oneshotRefinement}}{
%         \texttt{Refine Fun. ($ref.$)};
%     }
% \end{algorithm}

\subsection{Flexible Design Choice Configuration}
\begin{algorithm}[h]
\scriptsize
\caption{Execution flow of \algo.}
\label{alg:algo}
    \KwData{$p$ \tcp{Input point}}
    \KwData{$c$ \tcp{Temporal Clusters}}
    \KwData{$o$ \tcp{User's primary performance objective}}
    \KwData{$threshold$ \tcp{Identifying characteristics' changes}}
    \KwData{$queue$ \tcp{Batch of stream for detection}}
    \KwData{$struc.$ \tcp{Type of summarizing data structure}}   
    \KwData{$win.$ \tcp{Type of window model}}
    \KwData{$out.$ \tcp{Type of outlier detection mechanism}}
    \KwData{$ref.$ \tcp{Type of refinement strategy}}
    \tcp{Online Phase}
    Initializing parameters and design choices \;
    \While{!stop processing of input streams}{
      \eIf{\text{$queue$ is full}}{
            $struc._{old}$ = $struc.$ \;
            $characteristics$ = \texttt{Auto-detection Fun.(...)} \;
            $struc.$, $win.$, $out.$, $ref.$ = \texttt{Auto-selection Fun.(...)} \;
            \If{\text{$struc.$ != $struc._{old}$}}{
                Extract temporal clusters $c$ from old Summarizing Data Structure $s'$\;
                Initialize new Summarizing Data Structure $s$ based on $struc.$ and $c$\;
            }
            Empty $queue$ \;
        }{
            $queue$.push($p$) \;
        } 
        \texttt{Window Fun. (...)}\;
        \eIf{\text{$out.$ != \nod}}{
            $b$ $\gets$ \texttt{Outlier Fun. (...)}\;
            \If{\text{$b$ = false}}{
                \texttt{Insert Fun. (...)\tcp{Insert $p$ to $s$ and update $s$}}            
            }
        }{
            \texttt{Insert Fun. (...)\tcp{Insert $p$ to $s$ and update $s$}}
        }
        \If{\text{$ref.$ = \incrementalRefinement}}{
            \texttt{Refine Fun. ($ref.$)};
        }
    }
    \tcp{Offline Phase}
    \If{\text{$ref.$ = \oneshotRefinement}}{
        \texttt{Refine Fun. ($ref.$)};
    }
\end{algorithm}

The \emph{Window Fun.} (Algorithm~\ref{alg:algo_window}) applies different computing logic depending on the selected type of window models. The function maintains a counter $c$ to keep track of the number of processed data points and performs different actions based on the selected window model. 
\emph{Landmark Window} (Lines 4-8): If the \landmark window model is selected, the function checks whether the counter $c$ has exceeded the current landmark $m$. If so, the clustering results from the summarizing data structure $s$ are sunk (i.e., stored or output), and all clustering information is cleared. Then, the function updates the current landmark $m_{next}$ for the next window. This model is suitable for scenarios where data distributions change significantly over time, and the algorithm needs to adapt to these changes by periodically resetting the clustering information.
\emph{Damped Window} (Lines 9-10): In the \damped window model, the function updates the weights of data points and clusters in the summarizing data structure $s$ using the decay parameters $dc = (\alpha, \lambda)$. This model is designed for cases where older data points should have less influence on the clustering results. By applying a decay function, the algorithm can gradually forget outdated information and adapt to the current data distribution.
\emph{Sliding Window} (Lines 11-13): If the \sliding window model is chosen, the function checks whether the counter $c$ has exceeded the sliding window size $ws$. If so, the earliest data point in the window is removed from the summarizing data structure $s$. This model maintains a fixed-size window of the most recent data points, ensuring that the algorithm focuses on the current data distribution and disregards older data points that may no longer be relevant.

\begin{algorithm}[h]
\scriptsize
\caption{Window Fun. of \algo.}
\label{alg:algo_window}
    \SetKwFunction{FMain}{Window Fun.}
    \SetKwProg{Fn}{Function}{:}{}
    \tcc{$c$: counter (initialized with 0), $m$: landmark, $ws$: sliding window size, $dc = (\alpha, \lambda)$: decay parameters}
    \Fn{\FMain{$s$, $m$, $ws$, $dc$}}{
        $c$++\;
        \eIf{\text{$win.$ = \landmark }}{
            \If{\text{$c >$ $m$}}{
                Sink the clustering results from $s$\;
                Clear all of the clustering information\;
                $m$ $\gets$ $m_{next}$; \tcc{update current landmark}
            }                  
        }{\eIf{\text{$win.$ = \damped}}{
            Update weight with $dc$\;
            }(\tcp*[h]{\text{$win.$ = \sliding}}){
                \If{\text{$c >$  $ws$}}{
                    Remove the earliest point from window\;
                }                
            }        
               
        } 
    }    
\end{algorithm}

If outlier detection is enabled, the \emph{Outlier Fun.} (Algorithm~\ref{alg:algo_outlier}) is invoked. \emph{Outlier Fun.}  plays a crucial role in the outlier detection process of the \algo algorithm. It is responsible for detecting and managing outliers using different mechanisms based on the selected type of outlier detection ($out.$). The following is a more detailed explanation of the steps involved in the \emph{Outlier Fun.}:
\emph{Buffer Optimization} (Lines 2-8): If the selected outlier detection mechanism includes buffer or buffer with timer (\buffer or \buffertimer), the function checks if the input point ($p$) is an outlier. If $p$ is an outlier, it is inserted into the outlier buffer ($Buffer$) and assigned to the closest cluster ($cl$). The buffer cluster is then updated accordingly. After updating the cluster, the function checks if the cluster is dense enough (i.e., the density exceeds the specified threshold $d$). If the cluster is dense enough, it is moved from the outlier buffer to the summarizing data structure ($s$).
\emph{Regular Check} (Lines 9-24): The regular check is triggered at predefined intervals to assess the clusters in the summarizing data structure and the outlier buffer. For each cluster in the summarizing data structure, the function checks if the cluster is dense enough (density threshold $d$) and, if a timer-based mechanism is used (\timer or \buffertimer), if the cluster is active enough (timer threshold $t$). If a cluster is neither dense nor active, it is either moved to the outlier buffer (if enabled) or removed from the summarizing data structure.
\emph{Buffer Timer Check} (Lines 20-24): If the selected outlier detection mechanism is \buffertimer, the function checks the activity of each cluster in the outlier buffer based on the timer threshold ($t$). If a cluster in the buffer is not active, it is removed from the buffer.
\emph{Outlier Determination} (Line 25): The function returns whether the input point ($p$) is an outlier or not, based on the results of the previous steps.
By employing different outlier detection mechanisms, \algo is capable of efficiently handling various types of data streams and application requirements.

\begin{algorithm}[t]
\scriptsize
\caption{Outlier Fun. of \algo.}
\label{alg:algo_outlier}
    \SetKwFunction{FMain}{Outlier Fun.}
    \SetKwProg{Fn}{Function}{:}{}
    \tcc{$Buffer$: outlier buffers, $t$: timer threshold, $d$: density threshold}
    \Fn{\FMain{$p$, $s$, $Buffer$, $t$, $d$}}{ 
        \If{$out.$ = (\buffer \textbf{ Or } \buffertimer)}{
            \tcc{use buffer optimization}
            \If{($p$ Is Outlier) = true}{
                Select cluster $cl$ closest to $p$ from $Buffer$\;
                Insert $p$ to $cl$ and update $cl$\;
                bool $dense \gets$ Check ($cl$)\;
                \tcc{check if $cl$ is dense enough}
                \If{$dense$ = true}{
                    Move $cl$ from $Buffer$ to $s$\;
                }
            }
        }        
        \If{REGULAR CHECK TRIGGERED}{
            $cls \gets$ Extract($s$);\tcc{extract all clusters from $s$}
            \For{$cl \in cls$}{
                bool $active$ = false\;
                bool $dense \gets$ Check ($cl, d$)\;
                \tcc{check if $cl$ is dense enough}
                \If{$out.$ = (\timer \textbf{ Or } \buffertimer)}{
                    \tcc{use timer optimization}
                    bool $active \gets$ Check($cl.timer, t$)\;
                    \tcc{check if $cl$ is active enough }
                }
                \If{$dense$ = false \textbf{ and } $active$ = false}{
                    \If{BUFFER ENABLED}{
                        Insert $cl$ to $Buffer$\;
                    }
                    Remove $cl$ from $s$\; 
                }
            }   
            \If{\buffertimer}{
                \For{$cl \in Buffer$}{
                     bool $active \gets$ Check($cl.timer, t$)\;
                     \If{$active$ = false}{
                        Remove $cl$ from $Buffer$\; 
                    }
                }
            } 
        }
        Return ($p$ Is Outlier)\;
    }  
\end{algorithm}

The input point will then be added to the summarizing data structure if it is not identified as an outlier or if the algorithm does not use any outlier detection mechanisms.
In the \emph{Insert Fun.} (Algorithm~\ref{alg:algo_insert}), the input point $p$ is inserted into the summarizing data structure $struct.$. The function can adapt to different types of summarizing data structures, specifically those belonging to the hierarchical category and the partitional category. This adaptability of the \emph{Insert Fun.} allows \algo to effectively handle different types of summarizing data structures, catering to various needs and requirements. When the selected data structure belongs to the hierarchical category, the function inserts the input point $p$ into the appropriate cluster within the hierarchical data structure and updates the hierarchy accordingly (Lines 2-3). On the other hand, if the selected data structure belongs to the partitional category, the function first identifies the closest cluster for the input point $p$ and then inserts it into the identified cluster (Lines 4-5). After the insertion, the summarizing data structure is updated accordingly. 

\begin{algorithm}[h]
\scriptsize
\caption{Insert Fun. of \algo.}
\label{alg:algo_insert}
\SetKwFunction{FMain}{Insert Fun.}
\SetKwProg{Fn}{Function}{:}{}
\tcc{$p$: input, $struc.$: summarizing data structure}
\Fn{\FMain{$p$, $struc.$}}{
    \eIf{\text{$struc.$ belongs to hierarchical category}}{
    \tcc{Insert $p$ into the hierarchical data structure and update it}
        Insert $p$ into the appropriate cluster in the hierarchy;
        Update the hierarchy based on the insertion;
    }{
    \tcc{Insert $p$ into the partitional data structure and update it}
        Find the closest cluster for $p$;
        Insert $p$ into the closest cluster;
        Update the partitional data structure based on the insertion;
    }
}
\end{algorithm}

The \emph{Refine Fun.} (Algorithm~\ref{alg:algo_refine}) is responsible for refining the clustering results based on the selected refinement strategy ($ref.$). \algo provides two distinct refinement strategies: \incrementalRefinement and \oneshotRefinement, catering to different application requirements and data stream characteristics.
When \incrementalRefinement is applied, \algo continuously extracts the current clustering model from the summarizing data structure $s$. Then, it applies a suitable batch clustering algorithm to update the clustering model. After that, the function updates $s$ with the new clustering model and removes any outdated or redundant data points or clusters from $s$. This process ensures that the model remains up-to-date and adapts to the evolving data distribution.
When \oneshotRefinement is applied, it extracts all clusters and data points from the summarizing data structure $s$. It then applies a batch clustering algorithm to refine the clustering results. Finally, the function updates $s$ with the refined clustering results, providing a more accurate representation of the data distribution at the end of the processing. 

\begin{algorithm}[h]
\scriptsize
\caption{Refine Fun. of \algo.}
\label{alg:algo_refine}
\SetKwFunction{FMain}{Refine Fun.}
\SetKwProg{Fn}{Function}{:}{}
\tcc{$ref.$: Selected type of refinement strategy, $s$: Summarizing data structure}
\Fn{\FMain{$ref.$, $s$}}{
    \eIf{\text{$ref.$ = \incrementalRefinement}}{
        \tcc{Apply incremental refinement}
        Extract the current clustering model from $s$;
        Apply batch clustering algorithm to update the clustering model;
        Update $s$ with the new clustering model;
        Remove outdated or redundant data points or clusters from $s$;
    }{
        \tcc{Apply one-shot refinement}
        Extract all clusters and data points from $s$;
        Apply batch clustering algorithm to refine the clustering results;
        Update $s$ with the refined clustering results;
    }
}
\end{algorithm}



\subsection{Automatic Stream Characteristics Detection}
\begin{algorithm}[h]
\scriptsize
\caption{Auto-detection Func. of \algo}
\label{alg:auto_detection}
\SetKwFunction{FMain}{Auto-detection Func.}
\SetKwProg{Fn}{Function}{:}{}
\tcc{$batch$: a small batch of input stream data stored for detecting stream characteristic changes, $centers$: previous clustering centers of the stream data, $thresholds$: threshold values for identifying the characteristic}
\Fn{\FMain{$batch, centers, threshold$}}{
    \tcc{Initialize stream characteristics}
    \text{$characteristics$ = null}\;
    \text{$highDimData$ = $var$ = $numOfOutliers$= 0}\;
    \text{$samples$ = UniformSampling($batch$)}\;
    \text{$new\_center$ = mean($samples$)}\;
    \For{$s \in samples$}{
        \If{$s.dim  > thresholds.dim$}{
            $highDimData$ += 1 \;
        }
        $var$ = UpdateVariance($var, s, new\_centers$)\;
        $centers$ += $new\_center$ \;
        \If{$min(dist(s, centers))  > thresholds.dist$}{
            $numOfOutliers$ += 1 \;
        }
    }
    \eIf{$highDimData > num(samples) / 2$}{
        $characteristics.HighDimension = true$ \;
    }{
        $characteristics.HighDimension = false$ \;
    }
    \eIf{$var > thresholds.variance$}{
        $characteristics.HighConceptDrift = true$ \;
    }{
        $characteristics.HighConceptDrift = false$ \;
    }
    \eIf{$numOfOutliers > thresholds.outlier$}{
        $characteristics.ManyOutliers = true$ \;
    }{
        $characteristics.ManyOutliers = false$ \;
    }
    Return $characteristics$; 
}
\end{algorithm}

\subsection{Automatic Module Selection}
\begin{algorithm}[h]
\scriptsize
\caption{Auto-selection Func. of \algo}
\label{alg:auto_selection}
\SetKwFunction{FMain}{Auto-Selection Func.}
\SetKwProg{Fn}{Function}{:}{}
\tcc{$objective$: User's primary performance objective (Accuracy, Efficiency, or Balance); $data$: Input data stream; $characteristics$: Stream characteristics detected by auto-detect Func.}
\Fn{\FMain{$objective$, $data$, $characteristics$}}{
    \tcc{Initialize  four modular design components}
    \text{$struc.$= $win.$ = $out.$= $ref.$ = null}\;
    \eIf{$objective$ = Accuracy}{
        \tcc{Select modules with high accuracy based on input data stream characteristics}
        \eIf{$characteristics.HighConceptDrift = true$}{
            $struc.$ = \MCs \;
        }{
            $struc.$ = \MS \;
        }
        \eIf{$characteristics.ManyOutliers = true$}{
            $win.$ = \landmark \;
            $out.$ = \buffertimer \;
        }{
            $win.$ = \damped \;
            \eIf{$characteristics.HighDimension = true$}{
                $out.$ = \buffer \;
            }{
                $out.$ = \buffertimer \;
            }
        }
        $ref.$ = \incrementalRefinement \;
    }
    {
        \eIf{$objective$ = Efficiency}{
            \tcc{Choose a structure with high efficiency based on input data stream characteristics}
            \eIf{$characteristics.HighConceptDrift = true$}{
                $struc.$ = \DPT \;
                $win.$ = \landmark \;
            }{
                $struc.$ = \Grids \;
                $win.$ = \sliding \;
            }
            \eIf{$characteristics.ManyOutliers = true$}{
                $out.$ = \od \;
            }{
                $out.$ = \nod \;
            } 
            $ref.$ = \norefinement \;
        }{
            \tcc{Choose a structure with balanced accuracy and efficiency based on input data stream characteristics}
            \eIf{$characteristics.HighConceptDrift = true$}{
                $struc.$ = \CFT \;
            }{
                $struc.$ = \CoreT \;
            }
            $win.$ = \landmark \;
            $out.$ = \timer \;
            $ref.$ = \oneshotRefinement \;
        }
    }
    Return $struc.$, $win.$, $out.$, $ref.$; 
}
\end{algorithm}
% \subsection{Selecting Summarizing Data Structure}
% The SelectStructure function (Algorithm~\ref{alg:select_structure}) chooses the most suitable summarizing data structure based on the user's primary performance objective and the characteristics of the input data stream. Based on our observations, different summarizing data structures have different trade-offs between accuracy and efficiency. The function analyzes the input data stream to select the best structure that matches the user's preferences.

% If the user prefers accuracy, it selects a structure with high accuracy like \CoreT or \DPT. However, the function also considers the input data stream's characteristics to make a more informed decision. For example, if the input data has a high rate of change, \DPT may be more suitable due to its flexible updating mechanism.

% If the user prefers efficiency, it selects a structure with high efficiency like \CFT or \Grids. The function takes into account the input data stream's characteristics to select the most efficient structure for the given data. For example, if the input data has a low dimensionality and uniform distribution, \Grids might be a better choice due to its efficient distance calculation elimination.

% If the user seeks a balance between accuracy and efficiency, it selects a structure with balanced performance like \DPT or \CFT. The function considers the input data stream's characteristics to select the most suitable structure that provides a good balance between accuracy and efficiency.

% \begin{algorithm}[h]
% \scriptsize
% \caption{SelectStructure Function}
% \label{alg:select_structure}
% \SetKwFunction{FMain}{SelectStructure}
% \SetKwProg{Fn}{Function}{:}{}
% \tcc{$objective$: User's primary performance objective (Accuracy, Efficiency, or Balance); $data$: Input data stream characteristics}
% \Fn{\FMain{$objective$, $data$}}{
% \eIf{$objective$ = Accuracy}{
%     \tcc{Choose a structure with high accuracy based on input data stream characteristics}
%     \eIf{High rate of change in $data$}{
%         Return \DPT
%     }{
%         Return \CoreT
%     }
%     }{
%     \eIf{$objective$ = Efficiency}{
%     \tcc{Choose a structure with high efficiency based on input data stream characteristics}
%     \eIf{Low dimensionality and uniform distribution in $data$}{
%         Return \Grids
%     }{
%         Return \CFT
%     }
%     }{
%     \tcc{Choose a structure with balanced accuracy and efficiency based on input data stream characteristics}
%     \eIf{High rate of change in $data$}{
%         Return \DPT
%     }{
%         Return \CFT
%         }
%     }
%     }
% }
% \end{algorithm}

% \subsection{Selecting Window Model}

% The SelectWindowModel function (Algorithm~\ref{alg:select_window_model}) selects the most appropriate window model based on the user's primary performance objective and input data stream characteristics. Each window model has its strengths and weaknesses concerning accuracy and efficiency. The function takes into account both the user's preferences and the input data stream characteristics to select the most suitable window model.

% If the user prefers accuracy, it chooses a model with high accuracy like \landmark or \damped. The function also considers the input data stream's characteristics to make a more informed decision. For example, if the input data has a high rate of change, \damped may be more suitable due to its adaptive forgetting factor.

% If the user prefers efficiency, it chooses a model with high efficiency like \sliding. The function takes into account the input data stream's characteristics to select the most efficient window model for the given data. For example, if the input data has a relatively stable distribution, \sliding might be a better choice due to its fixed window size, which reduces the number of clusters for maintenance.

% If the user seeks a balance between accuracy and efficiency, it analyzes the input data stream and selects a suitable window model based on its characteristics and the desired balance. The function might choose \landmark or \damped for a balance favoring accuracy, or \sliding for a balance favoring efficiency. The specific choice would depend on the input data stream's characteristics and the desired balance of performance.

% \begin{algorithm}[h]
% \scriptsize
% \caption{SelectWindowModel Function}
% \label{alg:select_window_model}
% \SetKwFunction{FMain}{SelectWindowModel}
% \SetKwProg{Fn}{Function}{:}{}
% \tcc{$objective$: User's primary performance objective (Accuracy, Efficiency, or Balance); $stream$: Input data stream characteristics}
% \Fn{\FMain{$objective$, $stream$}}{
%     \eIf{$objective$ = Accuracy}{
%     \tcc{Choose a model with high accuracy based on input data stream characteristics}
%     \eIf{High rate of change in $stream$}{
%         Return \damped
%     }{
%         Return \landmark
%     }
%     }{
%     \eIf{$objective$ = Efficiency}{
%         \tcc{Choose a model with high efficiency based on input data stream characteristics}
%     \eIf{Stable distribution in $stream$}{
%         Return \sliding
%     }{
%         Analyze $stream$ and choose a suitable window model
%     }
%     }{
%         \tcc{Choose a suitable window model based on stream characteristics and balance}
%         Analyze $stream$ and select a window model that balances accuracy and efficiency
%     }
%     }
% }
% \end{algorithm}

% \subsection{Selecting Outlier Detection Mechanism}

% The SelectOutlierDetection function (Algorithm~\ref{alg:select_outlier_detection}) picks the best outlier detection mechanism based on the user's primary performance objective and input data stream characteristics. Each outlier detection mechanism has its strengths and weaknesses concerning accuracy and efficiency. The function takes into account both the user's preferences and the input data stream characteristics to select the most suitable outlier detection mechanism.

% If the user prefers accuracy, it chooses a mechanism with high accuracy like \buffer or \buffertimer. The function considers the input data stream's characteristics to make a more informed decision. For example, if the input data has a high rate of change, \buffertimer may be more suitable due to its combination of buffer and timer mechanisms, which can handle the evolving data distribution more effectively.

% If the user prefers efficiency, it chooses a mechanism with high efficiency like \timer. The function takes into account the input data stream's characteristics to select the most efficient outlier detection mechanism for the given data. For example, if the input data has a relatively stable distribution, \timer might be a better choice due to its lower maintenance overhead.

% If the user seeks a balance between accuracy and efficiency, it analyzes the input data stream and selects a suitable outlier detection mechanism based on its characteristics and the desired balance. The function might choose \buffer, \timer, or \buffertimer, depending on the input data stream's characteristics and the desired balance of performance. The specific choice would depend on the evolving nature of the input data stream and the user's tolerance for outlier detection errors.

% \begin{algorithm}[h]
% \scriptsize
% \caption{SelectOutlierDetection Function}
% \label{alg:select_outlier_detection}
% \SetKwFunction{FMain}{SelectOutlierDetection}
% \SetKwProg{Fn}{Function}{:}{}
% \tcc{$objective$: User's primary performance objective (Accuracy, Efficiency, or Balance); $stream$: Input data stream characteristics}
% \Fn{\FMain{$objective$, $stream$}}{
% \eIf{$objective$ = Accuracy}{
% \tcc{Choose a mechanism with high accuracy based on input data stream characteristics}
% \eIf{High rate of change in $stream$}{
% Return \buffertimer
% }{
% Return \buffer
% }
% }{
% \eIf{$objective$ = Efficiency}{
% \tcc{Choose a mechanism with high efficiency based on input data stream characteristics}
% \eIf{Stable distribution in $stream$}{
% Return \timer
% }{
% Analyze $stream$ and choose a suitable outlier detection mechanism
% }
% }{
% \tcc{Choose a suitable outlier detection mechanism based on stream characteristics and balance}
% Analyze $stream$ and select an outlier detection mechanism that balances accuracy and efficiency
% }
% }
% }
% \end{algorithm}

% \subsection{Selecting Refinement Strategy}

% The SelectRefinementStrategy function (Algorithm~\ref{alg:select_refinement_strategy}) selects the most suitable refinement strategy based on the user's primary performance objective and input data stream characteristics. If the user prefers accuracy, it chooses a strategy with high accuracy like \incrementalRefinement or \oneshotRefinement. If the user prefers efficiency, it may choose not to apply refinement. If the user seeks a balance between accuracy and efficiency, it analyzes the input data stream and selects a suitable refinement strategy based on its characteristics and the desired balance.

% The SelectRefinementStrategy function chooses the most suitable refinement strategy based on the user's primary performance objective and input data stream characteristics. The refinement strategies, such as \incrementalRefinement and \oneshotRefinement, can improve clustering accuracy but might affect the efficiency of the overall algorithm.

% If the user prefers accuracy, it chooses a strategy with high accuracy like \incrementalRefinement or \oneshotRefinement. The function considers the input data stream's characteristics to make a more informed decision. For example, if the input data has dynamic cluster formation, \incrementalRefinement may be more suitable due to its ability to adjust the clustering results iteratively.

% If the user prefers efficiency, it may choose not to apply any refinement strategy, as refinement can increase the computational cost and affect the overall efficiency of the algorithm.

% If the user seeks a balance between accuracy and efficiency, it analyzes the input data stream and selects a suitable refinement strategy based on its characteristics and the desired balance. The specific choice would depend on the input data stream's characteristics, the clustering algorithm's performance, and the user's tolerance for clustering errors. The function might choose \incrementalRefinement, \oneshotRefinement, or NoRefinement, depending on the input data stream's characteristics and the desired balance of performance.

% \begin{algorithm}[h]
% \scriptsize
% \caption{SelectRefinementStrategy Function}
% \label{alg:select_refinement_strategy}
% \SetKwFunction{FMain}{SelectRefinementStrategy}
% \SetKwProg{Fn}{Function}{:}{}
% \tcc{$objective$: User's primary performance objective (Accuracy, Efficiency, or Balance)}
% \tcc{$stream$: Input data stream characteristics}
% \Fn{\FMain{$objective$, $stream$}}{
%     \eIf{$objective$ = Accuracy}{
%         \tcc{Choose a strategy with high accuracy based on input data stream characteristics}
%         \eIf{Dynamic cluster formation in $stream$}{
%         Return \incrementalRefinement
%         }{
%         Return \oneshotRefinement
%         }
%     }{
%     \eIf{$objective$ = Efficiency}{
%         \tcc{Choose not to apply refinement for better efficiency}
%     Return NoRefinement
%     }{
%         \tcc{Choose a suitable refinement strategy based on stream characteristics and balance}
%         Analyze $stream$ and select a refinement strategy that balances accuracy and efficiency
%     }
%     }
% }
% \end{algorithm}

% \subsection{Decision Model}

% \textbf{Summarizing Data Structures.}
% In general, hierarchical summarizing data structure improves the clustering efficiency while the partitional structure is expected to bring better accuracy. The unique design of each specific structure, however, leads to further differences in their clustering behaviour. For example, although \CFT, \CoreT, \DPT, and \MCs promise high clustering accuracy due to the comprehensive information stored in their efficiency behaviour is quite different. Only \CFT and \DPT can guarantee high efficiency due to their flexible updating. \CoreT and \MS are slow due to frequently rebuilding the whole structure while \MCs is slow since it needs to scan every temporal cluster for data insertion. For \Grids, although it may not be as accurate as the other structures, it largely saves its computation time due to eliminating the distance calculation operation. 

% \textbf{Window Models.}
% Although these window models all try to prioritize the most recent data from streams, their specific strategies are quite different leading to different clustering behaviours. For a better clustering efficiency, \sliding may be the best choice since its fixed window size largely reduces the number of clusters for maintenance. On the contrary, although both \landmark and \damped may not be as efficient as the \sliding, they can bring in more accurate clustering results. Finally, for all three types of window models, their clustering behaviour is sensitive to their specific window configurations, which have not been studied in depth in the literature.

% \textbf{Outlier Detection Mechanisms.}
% The buffer and timer optimizations can be applied either separately or simultaneously, resulting in different decisions regarding the outlier detection mechanism. 
% The use of a buffer can greatly improve the clustering quality due to its better ability for handling \oef. However, maintaining the outlier buffer in real-time will also bring down the efficiency. 
% On the contrary, the use of the timer may be beneficial for both better clustering accuracy and efficiency, especially under \oef. 
% Using a buffer and timer together in outlier detection further complicates the clustering behaviour and motivates an in-depth study.

% \textbf{Refinement Strategies.}
% Refinement is optional and can be easily applied to refine online clustering results before outputting the result. The common wisdom is that it may further improve clustering quality. Unfortunately, there is no prior study about the real impact of this design aspect on both accuracy and efficiency. Even in recent years, some choose~\cite{StreamKM++:12} to involve this design aspect in their proposed \dsc algorithms, and some choose not~\cite{EDMStream:17}. We will empirically show its impact via extensive evaluations.

==> VLDB_block.tex <==

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
\endgroup
}
%%% VLDB block end %%%
